Multicalibrated Partitions for Importance Weights

The ratio between the probability that two distributions $R$ and $P$ give to points $x$ are known as importance weights or propensity scores and play a fundamental role in many different fields, most notably, statistics and machine learning. Among its applications, importance weights are central to domain adaptation, anomaly detection, and estimations of various divergences such as the KL divergence. We consider the common setting where $R$ and $P$ are only given through samples from each distribution. The vast literature on estimating importance weights is either heuristic, or makes strong assumptions about $R$ and $P$ or on the importance weights themselves. In this paper, we explore a computational perspective to the estimation of importance weights, which factors in the limitations and possibilities obtainable with bounded computational resources. We significantly strengthen previous work that use the MaxEntropy approach, that define the importance weights based on a distribution $Q$ closest to $P$, that looks the same as $R$ on every set $C \in \mathcal{C}$, where $\mathcal{C}$ may be a huge collection of sets. We show that the MaxEntropy approach may fail to assign high average scores to sets $C \in \mathcal{C}$, even when the average of ground truth weights for the set is evidently large. We similarly show that it may overestimate the average scores to sets $C \in \mathcal{C}$. We therefore formulate Sandwiching bounds as a notion of set-wise accuracy for importance weights. We study these bounds to show that they capture natural completeness and soundness requirements from the weights. We present an efficient algorithm that under standard learnability assumptions computes weights which satisfy these bounds. Our techniques rely on a new notion of multicalibrated partitions of the domain of the distributions, which appear to be useful objects in their own right.

==> algo_main.tex <==
\subsection{Algorithm for $(\alpha,\beta)$-multi-calibration}

We give an efficient algorithm  that computes a multicalibrated partition, given access to a weak agnostic learner for $\mC$. The algorithm is reminiscent of the algorithm for Boosting via Branching Programs due to \citep{mansour2002boosting}.  We first define weak agnostic learning. Given a collection of sets $\mC \subseteq 2^\X$, we can associate every set $C$ with its indicator function $c:\X \rgta \zo$. 

\begin{definition}
\label{def:weak-ag}
 A $(\alpha, \alpha', L)$-weak agnostic learning algorithm for a class $\mC$ is given $L$ samples from a distribution $\D = (\x, \y)$ where $\x \in \X$ and $\y \in \zo$. If there exists $c \in \mC$ such that $\Pr_\D{[c(\x) = \y}] \geq (1 + \alpha)/2$, then the learner will return $c' \in \mC'$ such that $\Pr_\D[c'(\x) = \y] \geq (1 + \alpha')/2$ for some $0 < \alpha' \leq \alpha$. The class $\mC$ is said to be $(\alpha, \alpha', L)$-weakly agnostically learnable if such a leaner exists. 
\end{definition}
We allow $\alpha - \alpha'$ to depend on $L$, typically it decreases with $L$. For simplicity, we will assume that $\mC' = \mC$, and do not allow for probability of error. 
\eat{

Given access to a weak agnostic learner, Algorithm \ref{alg:multiC} in Appendix \ref{sec:algorithms} efficiently finds an $(\alpha, \beta)$-\mcbd\ partition:

\begin{theorem}
 Given an $(\alpha, \alpha', L)$ weak agnostic learning algorithm for $\mC$, Algorithm \ref{alg:multiC} returns an $(\alpha, \beta)$-\mcbd\ partition for $\mC$ under $P,R$ within  $T$ iterations, where 
     $T =  \Tilde{O}(KL(R,P)/(\beta^2 \alpha'^4)$. 
    It makes $O(T)$ calls to the weak agnostic learner, where each call requires $\Tilde{O}(L /(\beta^2 \alpha'^2))$ samples from each of $R$ and $P$.

\end{theorem}
}

==> anomaly.tex <==
\section{Anomaly Detection}\label{sec:anomaly}

In anomaly detection, the ground truth scores $f^*(x)$ are derived from the importance weights $w^*(x) = R(x)/P(x)$ of $R$ relative to $P$. Common choices are  $f^*(x) = \log(w^*(x))$ or $f^*(x) = w^*(x)$. More generally, we can allow $f^* = g(w^*(x))$ for some sufficiently nice function $g$. Say that we have a multicalibrated partition $\mS$. Given that $w(x) = Q(x)/P(x)$ is our approximation to $w^*$, it is natural to hope that $f(x) = g(w(x))$ is a good approximation to $f^*(x)$. In this section we will show guarantees for this choice of $f$ when the underlying partition is multicalibrated.

We have argued that one cannot hope to identify anomalous points where $f(x)$ is large, rather the goal is to identify anomalous sets in a family of tests $\mC$. We say $C \in \mC$  is anomalous if  $R(C)/P(C)$ is large. In practice, typically there is some threshold $\tau$ for the anomaly score, above which a point is considered anomalous. One can hope that there is a set $C \in \mC$ that captures most points where $f^*(x) \geq \tau$. Choosing a `good' set of tests is the role of the practitioner. In this section we show that whenever there exits a set $C$ such that $g(R(C)/P(C))$ is large, then a random point sampled from $R|_C$ is given large weight by $f$, where the right notion of large is {\em at least $g(R(C)/P(C))$}. Additionaly we show that if there is a set $C$ that captures most of the `cleary normal' points, then multi-calibration implies a bound on the false positive rate.

It is interesting to observe that $\alpha$-multiAE  guarantees something weaker. Let $C$ be the set, assuming $w(x)$ are computed using an $\alpha$-multiAE partition, Equation~\eqref{eq:ae} shows that
\[
    \E_{x \sim P|_{C}}[w(x)] \in \E_{x \sim P|_{C}}[w(x^*)] \pm \frac{\alpha}{P(C)}.
\]
In other words, $\alpha$-multiAE guarantees that on average $w(x)$ is high, where the average is taken over $P$. Our goal however is to show that the average score is high under $R$, and for this multicalibration is required. 
\subsection{Logarithmic weights}

We start with the case when $g(t) = \log(t)$.  Our goal is to show that the average weight assigned to points from an anomalous set is large. Indeed, we can give a tight characterization of the expected anomaly score for every set $C \in \mC$. 

\begin{theorem}
\label{thm:omer}
    Under Assumptions \ref{asm:1} and \ref{asm:2}, for all $C \in \mC$ we have
    \begin{equation}
    \label{eq:exp-log}
        \llv\E_{\x \sim R|_C} [\log(w(x))] - \KL{Q|_C}{P|_C} - \logf{Q(C)}{P(C)}\rrv \leq   \gamma \frac{8\log(B)}{R(C)}.
    \end{equation}
    Hence for $C \in \mC$ such that $R(C) \geq 2\gamma$ we have
    \begin{equation}
    \label{eq:exp-log-lb}
        \E_{\x \sim R|_C} [\log(w(x))] \geq  \logf{R(C)}{P(C)} - \gamma \frac{8\log(B) + 2}{R(C)}.
    \end{equation}
\end{theorem}
\begin{proof}
    We first prove Equation \eqref{eq:exp-log}. We have
    \begin{align*}
        \E_{\x \sim R|_C} [\log(w(x))] & = \E_{\x \sim R|_C}\left[ \logf{Q(x)}{P(x)}\right] = \E_{\x \sim R|_C}\left[ \logf{Q|_C(x)Q(C)}{P|_C(x)P(C)}\right] \\
        &=  \E_{\x \sim R|_C}\left[ \logf{Q|_C(x)}{P|_C(x)}\right] + \logf{Q(C)}{P(C)}.
    \end{align*}
    We use this to derive Equation \eqref{eq:exp-log} as
    \begin{align*}
        \llv\E_{\x \sim R|_C} [\log(w(x))] - \KL{Q|_C}{P|_C} - \logf{Q(C)}{P(C)}\rrv  
        &\leq  \llv\E_{\x \sim R|_C}\left[ \logf{Q|_C(x)}{P|_C(x)}\right] - \E_{\x \sim Q|_C}\left[\logf{Q|_C(x)}{P|_C(x)}\right]\rrv\\
        &\leq \frac{8\gamma \log(B)}{R(C)}
    \end{align*}
    where the last inequality follows by applying Theorem \ref{thm:exp-bound} and using  $\infnorm{Q|_C/P|_C} \leq B^2$.

    We now derive Equation \eqref{eq:exp-log-lb} from it. We have
    \begin{align}
        \llv \logf{Q(C)}{P(C)} - \logf{R(C)}{P(C)}\rrv &= 
        \llv\logf{Q(C)}{R(C)}\rrv = \llv\log\left(1 + \frac{Q(C) - R(C)}{R(C)}\right)\rrv \notag\\
        &\leq  \frac{2|Q(C) - R(C)|}{R(C)} \leq \frac{2\gamma}{R(C)}\label{eq:q-vs-p}
    \end{align}
    where we  use $|\log(1 + x)| \leq 2|x|$ for $|x| \leq 1/2$, which applies since we assume $R(C) \geq 2\gamma$, so 
    \[ \frac{|Q(C) - R(C)|}{R(C)} \leq \frac{\gamma}{R(C)} \leq 1/2.\]
    
    From Equation \eqref{eq:exp-log}, we have 
    \begin{align*}
        \E_{\x \sim R|_C} [\log(w(x))] &\geq \KL{Q|_C}{P|_C}  + \logf{Q(C)}{P(C)} - \frac{8 \log(B)}{R(C)}\\
        &\geq \logf{R(C)}{P(C)} - \gamma \frac{8\log(B) + 2}{R(C)}
    \end{align*}
    where in the last line we use the positivity of KL divergence and Equation \eqref{eq:q-vs-p}.
\end{proof}


\subsection{Polynomial anomaly scores}

Next we consider the case where $g(t) = t$. In this case, we can characterize the expected anomaly scores in terms of the Renyi $2$-divergence. For any $\theta > 0$, the Renyi $1 + \theta$-divergence is defined as
\begin{equation}
    \label{eq:def-renyi}
    \ren{1 + \theta}{Q}{P} = \frac{1}{\theta}\log\left(\E_{\x \sim Q}\left[\left(\frac{Q(\x)}{P(\x)}\right)^\theta\right]\right).
\end{equation}

\begin{lemma}
\label{lem:exp-lin}
    Under Assumptions \ref{asm:1} and \ref{asm:2}, for all $C \in \mC$ 
    \begin{equation}
    \label{eq:exp-lin}
        \llv\E_{\x \sim R|_C} [w(x)] - \frac{Q(C)}{P(C)}\exp(\ren{2}{Q|_C}{P|_C}) \rrv \leq   \gamma \frac{8B}{R(C)}.
    \end{equation}
\end{lemma}
\begin{proof}
    Since $\infnorm{w(x)} \leq B$, we can apply Theorem \ref{thm:exp-bound} to get
    \begin{align}
     \llv\E_{\x \sim R|_C}[w(x)] - \E_{\x \sim Q|_C}[w(x)] \rrv \leq \frac{8\gamma B}{R(C)} .\label{eq:first_part}
    \end{align}
    We have
    \begin{align*}
        \E_{\x \sim Q|_C} [(w(x))] &= \E_{\x \sim Q|_C}\left[ \frac{Q(x)}{P(x)}\right]
        =  \E_{\x \sim Q|_C}\left[ \frac{Q|_C(x)}{P|_C(x)}\right] \frac{Q(C)}{P(C)}\\
        & = \exp\left(\ren{2}{Q|_C}{P_C}\right)\frac{Q(C)}{P(C)}.
    \end{align*}
\end{proof}

To see the similarity to  Theorem \ref{thm:omer}, we need take logarithms. This is somewhat complicated by the fact that we have additive error in Equation \eqref{eq:exp-lin}. For intuition, we assume that the error term $\gamma B/R(C)$ is small enough  compared to  $\E_{\x \sim R|_C} [w(x)]$ so that we can ignore it, hence
\begin{equation*}
    \E_{\x \sim R|_C} [w(x)] \approx \frac{Q(C)}{P(C)}\exp\left(\ren{2}{Q|_C}{P|_C}\right).
\end{equation*}
Now taking logarithms on either side, 
\begin{align}
    \label{eq:d2}
    \log\left(\E_{\x \sim R|_C} [w(x)]\right) \approx \logf{Q(C)}{P(C)} + \ren{2}{Q|_C}{P|_C}.
\end{align}
Note the similarity between these bounds and Equations \eqref{eq:exp-log}. By the positivity of Renyi divergence, we can then derive a lower bound similar to \eqref{eq:exp-log-lb}, we do this formally in Corollary \ref{cor:tech} in the next section. A similar analysis can be performed for $g(t) = t^\theta$ for any $\theta > 0$, to get the following conclusion:
\begin{align}
\label{eq:dtheta}
    \frac{1}{\theta}\log\left(\E_{\x \sim R|_C} [w(x)]\right) &\approx \logf{Q(C)}{P(C)} + \ren{1 + \theta}{Q|_C}{P|_C}.
\end{align}

\subsection{A lower bound for general anomaly scores}

Generalizing this, we consider anomaly scores of the form $f(x) = g(w(x))$ any monotone, univariate function $g:\R \rgta \R$ such that $t\cdot g(t)$ is convex; this includes $\log(t)$ and $t^\theta$ for any $\theta > 0$. 

\begin{lemma}
\label{lem:tech}
     Let $g: \R \rgta \R $ be a monotone, $L$-Lipschitz function on the range $[1/B, B]$ such that $tg(t)$ is convex. Let $f(x) = g(w(x))$ and $G = \max(|g(B)|, |g(1/B)|)$.
     Then under Assumptions \ref{asm:1} and \ref{asm:2}, for all $C \in \mC$ we have
    \begin{align*}
        \E_{\x \sim R|_C}[f(\x)]  \geq g\left(\frac{R(C)}{P(C)}\right) - \frac{8\gamma G}{R(C)} - \frac{\gamma L}{P(C)} .
    \end{align*}
\end{lemma}


The proof appears in Appendix \ref{app:general_anomaly}. Specializing to the case $g(t) = t^\theta$ for $\theta > 0$, where $G \leq B^\theta$ and $L \leq \theta B^{\theta -1}$ we have:
\begin{corollary}
\label{cor:tech}
     Let $f(x) = w(x)^\theta$ for $\theta > 0$.
     Then under Assumptions \ref{asm:1} and \ref{asm:2}, for all $C \in \mC$ 
     \begin{align*}
        \E_{\x \sim R|_C}[w(\x)^\theta]  \geq \left(\frac{R(C)}{P(C)}\right)^\theta - \frac{8\gamma B^\theta}{R(C)} - \frac{\gamma \theta B^{\theta -1}}{P(C)} .
    \end{align*}
\end{corollary}


\eat{



\begin{corollary}
\label{cor:anomaly}
Let $C$ be such that $R(C) \geq 4\gamma$. Under Assumption \ref{asm:1} and the boundedness assumption,
    \[ \sum_{x \in C} R(x)\log(w(x))  \geq  (R(C) - \gamma)\log\left(\frac{R(C)}{P(C)}\right) - 4\gamma(\log(B) +1).\]
\end{corollary}
\begin{proof}
    Since $f(x) = \log(w(x)) \in \mFS$, Lemma \ref{lem:omer} implies that 
    \begin{align}
        \label{eq:lb1}
         \sum_{x \in C} R(x)\log(g(w(x)))  \geq \sum_{x \in C} Q(x)f(x) - \alpha \E_{\x \sim R}[|f(\x)|] - \beta \|f\|_\infty.
    \end{align}
    By Lemma \ref{lem:tech} and using $Q(C) \geq R(C) - \gamma$,
    \begin{align*} 
    \sum_{x \in C} Q(x)\log(w(x)) &\geq Q(C)\logf{Q(C)}{P(C)} \geq (R(C) - \gamma)\logf{R(C) - \gamma}{P(C)}\\
        &= (R(C) -\gamma)\logf{R(C)}{P(C)} + (R(C) - \gamma)\log\left(1 - \frac{\gamma}{R(C)}\right)\\
        &\geq (R(C) -\gamma)\logf{R(C)}{P(C)} + (R(C) - \gamma)\frac{-2\gamma}{R(C)}\\
        & \geq (R(C) -\gamma)\logf{R(C)}{P(C)} - 2\gamma 
    \end{align*}
    where we use the inequality $\log(1 - x) \geq - 2x$ which holds when $x \in (0,1/4]$.
    For the second term, 
    \begin{align*} 
    \E_{\x \sim R}[|f(\x)|] = \E_{\s \sim R^\mS}[|f(\s)|] = \sum_{S \in \mS} R(S) \abs{\logf{R(S)}{P(S)}} \leq 2 + \KL{R^\mS}{P^\mS}.
    \end{align*}
    For the last term we, plug in $\infnorm{f} = \infnorm{\log(w)}$. Substituting into Equation \eqref{eq:lb1}, 
    \begin{align*}
         \sum_{x \in C} R(x)\log(g(w(x)))  &\geq  (R(C) -\gamma)\logf{R(C)}{P(C)} - \gamma - \alpha(2 + \KL{R^\mS}{P^\mS}) - \beta \infnorm{\log(w)}\\ 
        &\geq  (R(C) - \gamma)\log\left(\frac{R(C)}{P(C)}\right) - \alpha\KL{R^\mS}{P^\mS} - \beta \infnorm{\log(w)} -4\gamma.
    \end{align*}
\end{proof}
}



\subsection{Bounded false-positive rate} Probably the greatest pain point of anomaly detection algorithms in practice is a high rate of false positives. In this section we show that multi-calibration implies a bound on the false positive rate of anomaly reporting.

Recall that the points with high importance weights are marked as anomalous, and therefore let all the points in the highest state $S$ be marked as being anomalous. Our result holds under the condition that the hypothesis class $\mC$ captures the set of clearly normal points which we do not want to mark as anomalous. Under this condition, we show that $(\alpha,\beta)$-multicalibration implies that only a small fraction of non-anomalous points are contained in $S$ as long as $R(S)\ge \beta$ (note that if $R(S)$ is very small, then the fraction reported as anomalies is itself small and hence the false positive rate is not a major concern). The proof appears in Appendix \ref{app:false_positive}.

%Let $\tau$ be a threshold above which we consider a point to be an anomaly. Let $\delta > 0$ and $ C = \{ x: w^*(x) \leq \tau - \delta\}$. The set $ C$ could be thought of as the set of clearly normal points, these are points we do not want to mark as anomalies. We assume $ C \in \mathcal C$ which captures the case the clearly normal points are identified by the model. We will assume for convenience that $\beta = 0$ and that $R(C)$ is greater than $1/2$. Now let $S$ be the part of the partition such that $\frac{R(S)}{P(S)} \geq \tau$. Note that we assume for convenience that the partition breaks off exactly at $\tau$. Since points in $S$ are reported as anomalies,  $C\cap S$ are false positives and the false positive rate is $\frac{R(C\cap S)}{R(S)}$. 

\begin{theorem}
Let $\tau$ be a threshold above which we consider a point to be an anomaly and let $S$ be the state marked as anomalous, therefore $\frac{R(S)}{P(S)} \geq \tau$. Let  $\delta > 0$ and $ C = \{ x: w^*(x) \leq \tau - \delta\}$ be the set of clearly normal points. Assume $C\in \mC$, and $R(C)\ge 1/2$. Then under Assumption \ref{asm:1} with $R(S)\ge \beta$, the false positive rate $\frac{R(C\cap S)}{R(S)}$ is bounded as,
\[
\frac{R(C\cap S)}{R(S)} \leq \frac{2\tau\gamma}{\delta} + \frac{4\gamma}{R(S)}.
\]
\end{theorem}\label{thm:false_positive}



==> app_proofs.tex <==
\section{Additional Proofs}

\subsection{Properties of Boundedness}\label{app:bounded}

We note some simple properties of $\infnorm{P/R}$.
\begin{lemma}
Let $\mS$ be a partition of $\X$. Let $P$ and $R$ be distributions on $\X$ and $Q$ be the reweighted distribution.     \begin{gather}
        \forall A \subseteq \X, \  \ \frac{R(A)}{P(A)} \leq \infnorm{R/P} \label{eq:cons-1},\\
        \infnorm{Q/P} \leq \infnorm{R/P}, \infnorm{P/Q} \leq \infnorm{P/R} \label{eq:cons-2},\\
        \forall A \subseteq \X, \ \ \max(\infnorm{Q|_A/P|_A}, \infnorm{P|_A/Q|_A}) \leq \infnorm{R/P}\infnorm{P/R}. \label{eq:cons-3}
    \end{gather}
\end{lemma}
\begin{proof}
    Equation \eqref{eq:cons-1} follows from
    \[\frac{R(A)}{P(A)} = \frac{\sum_{x \in A} R(x)}{\sum_{x \in A} P(x)} \leq \max_{x \in A} \frac{R(x)}{P(x)} .\]
    For Equation \eqref{eq:cons-2} we observe that for $S \ni x$, 
    \[ \frac{Q(x)}{P(x)} = \frac{R(S)}{P(S)} \leq \infnorm{R/P}, \frac{P(x)}{Q(x)} = \frac{P(S)}{R(S)} \leq \infnorm{P/R} . \]
    For Equation \eqref{eq:cons-3},  for $S \ni x$
    \[ \frac{Q|_A(x)}{P|_A(x)} = \frac{Q(x)}{P(x)}\frac{P(A)}{Q(A)} \leq \infnorm{R/P}\infnorm{P/R}. \]
    where we use the Equations \eqref{eq:cons-2} and \eqref{eq:cons-1}. A similar bound holds for its reciprocal. 
\end{proof}

\subsection{Proof of Theorem \ref{thm:pyth3}}\label{app:weaken_bounded_proof}

The proof of Theorem \ref{thm:pyth3} uses the following lemma.

\begin{lemma}
\label{lem:kl-abs}
    For any two distributions $U, V$ on a domain $\X$,
    \[ E_{\x \sim U}\left[\abs{\logf{U(\x)}{V(\x)}}\right] \leq \KL{U}{V} + 2.\] 
\end{lemma}



We now give the proof of Theorem \ref{thm:pyth3}. 

\begin{proof}[Proof of Theorem \ref{thm:pyth3}]
We have
\begin{align}
\label{eq:part1}
    R(C)(\KL{R|_C}{P|_C} - \KL{R|_C}{P|_C}) &= R(C)\sum_{x \in C}\frac{R(x)}{R(C)} \left(\logf{R(x)P(C)}{R(C)P(x)} - \logf{R(x)Q(C)}{R(C)Q(x)} \right)\notag\\
    &= \sum_{x \in C}R(x)\logf{Q(x)P(C)}{Q(C)P(x)},\\
    Q(C)\KL{Q|_C}{P|_C} &= \sum_{x \in C} Q(x)\logf{Q(x)P(C)}{Q(C)P(x)}.\label{eq:part2}
\end{align}
Subtracting Equation \eqref{eq:part2} from \eqref{eq:part1}, since $Q(x)/P(x) = R(S)/P(S)$ for $x \in S$, we can write
\begin{align}
    \label{eq:rewrite}
    R(C)(\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C}) - Q(C)\KL{Q|_C}{P|_C} 
    = \sum_{S \in \mS}\sum_{x \in C} (R(x) - Q(x))\logf{R(S)P(C)}{Q(C)P(S)}\notag\\
    = \sum_{S \in \mS} (R(S \cap C) - Q(S \cap C))\left( \logf{R(S)}{P(S)} + \logf{P(C)}{Q(C)}\right).
\end{align}

We bound the absolute values of the two sums separately. For the first, we apply Lemma \ref{lem:omer}. By the $B$-boundedness assumption, and Lemma \ref{lem:kl-abs} respectively,
\begin{align*} 
    \max_{S \in \mS} \logf{R(S)}{P(S)}  & \leq \log(B), \\
    \E_{\s \sim \R^\mS}\abs{\logf{R(\s)}{P(\s)}} & \leq \KL{R^\mS}{P^\mS} + 2.
\end{align*}
Plugging these bounds into Lemma \ref{lem:omer},
\begin{align}
    \label{eq:term1}
    \abs{\sum_{S \in \mS} (R(S \cap C) - Q(S \cap C))\logf{R(S)}{P(S)}} &\leq 
    \alpha (\KL{R^\mS}{P^\mS} + 2) + \beta\log(B).
\end{align}
We bound the second term as
\begin{align}
    \label{eq:term2}
     \abs{\sum_{S \in \mS} (R(S \cap C) - Q(S \cap C))\logf{P(C)}{Q(C)}} &\leq \abs{(R(C) - Q(C))}\abs{\logf{P(C)}{Q(C)}} \notag\\
     & \leq \gamma \abs{\logf{P(C)}{Q(C)}}.
\end{align}
Plugging Equations \eqref{eq:term1} and \eqref{eq:term2} back into Equation \eqref{eq:rewrite} and dividing by $R(C)$ gives Equation \eqref{eq:p-approx}.
\end{proof}

\subsection{Proof of Lemma \ref{lem:tech}}\label{app:general_anomaly}

\begin{proof}
Since $g$ is monotone, we have 
\[ \infnorm{f(x)} = \infnorm{g(w(x))} \leq \max(|g(B)|, |g(1/B)|) = G. \]
Since $f \in \mFS$, and $\infnorm{f} \leq G$, by Theorem \ref{thm:exp-bound}
\begin{align}
    \label{eq:q-lb}
     \E_{\x \sim R|_C}[f(\x)] \geq \E_{\x \sim Q|_C}[f(\x)]  -  \frac{8\gamma G}{R(C)}.
\end{align}
We now lower bound  $\E_{\x \sim Q|_C}[f(\x)]$. Since $Q(x) = P(x)w(x)$, we can write
    \begin{align}
        \E_{\x \sim Q|_C}[f(\x)] &= \frac{1}{Q(C)}\sum_{x \in C} P(x)w(x)g(w(x)\notag\\
        &= \frac{P(C)}{Q(C)}\left(\E_{\x \sim P|_C}[w(x)g(w(x))]\right)\notag\\
        & \geq \frac{P(C)}{Q(C)} \left( \E_{\x \sim P|_C}[w(x)]\right)g\left( \E_{\x \sim P|_C}[w(x)]\right) \hspace{2cm} \text{(convexity of} \ tg(t))\notag\\
        & = \frac{P(C)}{Q(C)} \frac{Q(C)}{P(C)}g\left( \frac{Q(C)}{P(C)}\right)\notag\\
        & \geq g\left(\frac{R(C)}{P(C)}\right) - \frac{\gamma L}{P(C)}. 
    \end{align}
    where the last inequality holds by the Lipshcitz property, since $|Q(C) - R(C)| \leq \gamma$, 
    Plugging this into Equation \eqref{eq:q-lb}  completes the proof. 
\end{proof}

\subsection{Proof of Theorem \ref{thm:false_positive}}\label{app:false_positive}

\begin{proof}
Since $R(S)\ge \beta$, it is multi-calibrated and we can apply the guarantee in Equation~\eqref{eq:multic} to get,
%By Equation~\eqref{eq:multic},
\begin{align*}
    P(C\cap S) \abs{ \E_{x \sim P(C\cap S)} [w^*] - \frac{R(S)}{P(S)} } \leq \gamma R(S).
\end{align*}
Since $\frac{R(S)}{P(S)} \geq \tau$ and $E_{x \sim P(C\cap S)} [w^*]\le \tau-\delta$, this implies that 
\begin{align}
    P(C\cap S) \leq \frac{\gamma R(S)}{\delta}.\label{eq:fp1}
\end{align}

We now instantiate Theorem~\ref{thm:exp-bound} with $f$ the indicator of  $S$.
\[
\frac{R(C \cap S)}{R(C)} \leq \frac{Q(C \cap S)}{Q(C)} + \frac{4\gamma}{R(C)}.
\]
Since
\begin{align*}
    \frac{Q(C \cap S)}{Q(C)} &= \frac{R(S)P(C|S)}{Q(C)}= \frac{R(S)P(C\cap S)}{Q(C)P(S)}\\
    &\le \frac{\tau P(C\cap S)}{Q(C)}.
\end{align*}
Therefore
\begin{align}
R(C\cap S) &\leq \tau \frac{R(C)}{Q(C)}P(C\cap S) + 4\gamma \nonumber\\
\implies \frac{R(C\cap S)}{R(S)} &\leq \tau \frac{R(C)}{Q(C)}\cdot \frac{P(C\cap S)}{R(S)} + \frac{4\gamma}{R(S)}.\label{eq:fp2}
\end{align}
Now, by $\gamma$-multiAE and since $R(C)\ge 1/2$,
\begin{align*}
    \frac{R(C)}{Q(C)} \le \frac{R(C)}{R(C)-\gamma} \le \frac{1}{1-2\gamma}\le 2.
\end{align*}
Using this in Equation \eqref{eq:fp2} along with the bound from Equation \eqref{eq:fp1} we get a bound on the probability of a false positive:
\[
\frac{R(C\cap S)}{R(S)} \leq \frac{2\tau\gamma}{\delta} + \frac{4\gamma}{R(S)}.
\]

\end{proof}
\eat{
\subsection{Proof of Theorem \ref{thm:maxent}}\label{app:multiaccuracy}

\begin{proof}
    If at iteration $T$ the weak learner fails to find $C \in \mC$ where $|R(C) - Q_T(C)| \geq \alpha'$, it must hold that $|R(C') - Q_T(C')| \leq \alpha$ for every $C' \in \mC$, hence $Q_T$ is $\alpha$-mulitaccurate. 
    
    To prove termination, we show that $\KL{R}{Q_t}$ decreases in every step. For any $t \geq 1$, 
    \begin{align}
        \KL{R}{Q_t} - \KL{R}{Q_{t+1}} &= \sum_{x \in \X}R(x)\logf{Q_{t+1}(x)}{Q_t(x)}\notag\\
        &= \sum_{x \in \X}R(x)\logf{\exp(\eta c_t(x))}{\E_{\x \sim Q_t}[\exp(\eta c_t(\x))]}\notag\\
        &= \logf{1}{\E_{\x \sim Q_t}[\exp(\eta c_t(\x))]} + \sum_{x \in \X} R(x)\eta c_t(x)\notag\\
        &= -\log\left(\E_{\x \sim Q_t}[\exp(\eta c_t(\x))]\right) + \eta R(C_t). \label{eq:kl-prog}
    \end{align}

We now lower bound the first term. Since $\eta \leq 1/2$ and $c_t(x) \in \zo$ we have
\begin{align*}
        \exp(\eta c_t(x)) \leq 1 + \eta c_t(x) + \eta^2.
    \end{align*}
    Taking expectations under $Q_t$, 
    \begin{align*}
        \E_{\x \sim Q_t} [\exp(\eta c_t(\x))] \leq 1 + \eta \E_{\x \sim Q_t} [c_t(x)] + \eta^2 = 1 + \eta Q_t(C_t) + \eta^2.
    \end{align*}
    Since $\eta \leq 1/2$,  $\eta Q_t(C_t) + \eta^2 \leq 1$. Since $\log(1 + x) \leq x$ when $x \in[0,1]$, we have
    \begin{align}
        \label{eq:term1}
        -\log\left(\E_{\x \sim Q_t}[\exp(\eta c_t(\x))]\right) \geq -\log(1 + \eta Q_t(C_t) + \eta^2) \geq -\eta Q_t(C_t) - \eta^2.
    \end{align}
    Plugging this into Equation \eqref{eq:kl-prog} 
    \begin{align*}
        \KL{R}{Q_t} - \KL{R}{Q_{t+1}} = \eta(R(C_t) - Q_t(C_t)) -\eta^2 \geq \eta\alpha' -\eta^2 = \alpha'^2/4.
    \end{align*}
    Since we start at $Q_1 = P$ and each step reduces the KL divergence by $\alpha'^2/4$ the number of iterations is bounded by $T = 4\KL{R}{P}/\alpha'^2$.
\end{proof}
}

==> applications.tex <==
\section{Applications of multicalibration}

==> arxiv/old/intro_old.tex <==
\section*{Introduction (Old)}

Consider a scenario where we are observing samples drawn from a distribution $R$ over some domain $\X$. The domain $\X$ might represent demographic information of people, whereas $R$ might be the distribution of people who voted, who applied to college or were afflicted with the flu virus. We have some knowledge about the distribution, perhaps from previous experience, which is captured by a prior distribution $P$. While $P$ is probably a good baseline, we do not expect it to be a perfect model for $R$. How can we modify $P$ to better represent $R$, as opposed to building a new model from scratch? This question arises both in supervised and unsupervised learning. It is core to the study  of domain adaptation or transductional learning in supervised setting, and density-ratio estimation and anomaly detection in the unsupervised setting (this particular flavor is sometimes referred to as semi-supervised learning).

The statistical technique of importance weighting, also called density ratio estimation provides an approach to this problem. For each $x \in \X$, let us define its importance weight under $R$ to be $w_R(x) = R(x)/P(x)$. This defines a function $w_R: \X \rgta \R^+$. Learning this function is the key goal of density ratio estimation. If we have a closed form for the probability density function (pdf) of $P$, then $P(x)w_R(x)$ is a closed form for the pdf of $R$. If we only have random samples from $P$, knowing $w_R$ suffices to generate random samples from $R$ using importance sampling. Indeed, in several applications including anomaly detection and divergence estimation, learning the weights $w_R$ is sufficient, and is potentially easier than learning both $P$ and $R$.  

Learning $w_R$ exactly from random samples alone is not feasible, without some strong assumptions on the distributions themselves. Intuitively, it is clear that for continuous distributions (or discrete distributions with large support), one cannot hope to give accurately compute $w_R(x)$ for all $x \in \X$ from a small number of samples. One could ask if the issue is merely that of sample complexity. For large sets $S$, could one hope that the average importance weight assigned to a point within $S$ is accurate, in analogy with calibration for predictors? However, the barriers are also computational. Assuming one-way functions exist, there exists distributions on $\zo^n$ and sets $S$ for which it is hard to tell if $r(S)/p(S) \approx 0$  or $r(S)/p(S) = 1$. One needs to assume some computational niceness about the sets $S$ to be able to have even such average-case guarantees. 


Indeed, a popular way  to deal with this is the functional approximation route, where we come up with an approximation $w_Q$ of $w_R$ lying in a structured class of functions, over which optimization is efficient. The guarantee is typically that $w_Q$ is close to the best approximation to $w_R$ within the structured class. 

In this work, we take a different approach inspired by recent work on fairness. We fix a large family of statistical tests  $\mH$ specified by subsets of $\X$. The computational requirement of our family $\mH$ is that we can perform Empirical Risk Minimization (ERM) over it.
Given the difficulty of point-wise approximation, one might hope for {\em average case guarantees}, where for all subsets $S \subset \mH$, the importance weights are correct for points in the set on average. We will go a step further and ask for a stronger guarantee where for each set $S$ in the family, over points in $S$ where our estimator assigns the importance weight $w$, the average is indeed close to $w$. This is similar to requiring that our estimator of importance weights is multicalibrated for sets in $\mH$. This is analogous to the situation in fairness, where individual fairness is often hard to achieve, but several meaningful  notions of group fairness are feasible. 

We show that this definition is achievable, by giving an algorithm that achieves multi-calibration, using an ERM subroutine for $\mH$. We show that the resulting importance weights are useful for several applications including anomaly detection, divergence estimation and transfer learning. 

==> arxiv/old/old-prelims.tex <==
\
Our goal, given samples from $R$ and $P$ is to learn a model $Q$ for $R$ such that $Q$ is a good approximation to $R$. Our notion of good approximation is with regard to a family of statistical tests $\mC = \{S \subseteq \X\}$. 



This suggests computational and size restrictions to be placed on the family of sets for which we hope to give guarantees:
\begin{itemize}
    \item The sets should be computationally simple. At the very least, one should be able to tests membership in the set efficiently. 
    \item The sets should be large. If either $R(A)$ is too small, one cannot hope to test whether $\|R(A) - Q(A)\|$ is small with low sample complexity. 
\end{itemize}
Given $A \subseteq \X$ such that both conditions hold, we can get a multiplicative estimate for $w_R(A)$ from random sampling, provided $R(A)$ and $P(A)$ are not too small: we simply estimate $R(A)$ and $P(A)$ from random samples using the membership test, and take their ratio.  For such a set, if someone were to present us with a distribution $Q$ or its importance weight function $w_Q$, we can test whether $Q(A)$ and $R(A)$ are close. 


Our goal will be to simultaneously approximate $R(A)$ for a (possibly infinite) family of sets $A \in \mA$; $\mA$ could be all neural nets of a certain size, or decision trees of a certain depth. 
\begin{definition}
    An weight function $w_Q$  is said to be $\eps$-multiaccurate for $w_R$ with regard to $\mA$ if the distribution $Q(x) = q_Q(x)P(x)$ $ satufies the following condition for every $A \in \mA$ 
    \[ Q(A) =  R(A) \pm \eps. \]
    
    An importance weight function $w_Q$  is said to be $(\mu, \delta)$-calibrated for $w_R$ with regard to $\mA$ if for every $A \in \mA$ such that $P(A) \geq \mu, R(A) \geq \mu$, it holds that
\end{definition}



The key to achieving such a simultaneous approximation is the following notion 
\begin{defintion}
    A partition $\Y = \{y_1, \ldots, y_w\}$ of $\X$ is $\delta$-calibrated for $\H$ if for every $A \in \H$, if $$
\end{defintion}


Our approach will rely on forming partitions of the space $\X$ such that points within the each set in  the partition have nearly equal importance weights.  The following construction, which is computationally inefficient illustrates the idea behind this approach. 
Abusing notation, for $x \in \X$ we will write $w(x) = R(x)/P(x)$ rather than $w(\{x\})$. The following construction partitions space based on the importance weights $w(x)$ for each individual point $x \in X$. 
\begin{lemma}
    \label{lem:exist}
    Assume that $R, P$ are distributions on $\X$ such that for all $x \in  \supp(P)\cup \supp(R)$,
    \[ \max\left(\frac{R(x)}{P(x)}, \frac{P(x)}{R(x)}\right) \leq B. \]
    There exists a partition $\Y = \{y_1, \ldots, y_m\}$ of $\X$ such that $m \leq O(\log(B)/\delta)$
    and for every $A \subseteq \X$, $w(A \cap y) = w(y)( 1 \pm \delta)$. 
\end{lemma}
\begin{proof}
    Note that $w(x) \in [1/B, B]$. We partition this range into geometric scales of $(1 + \delta)$ and place the $x$s where $w(x)$ lies in a scale in the same $y_j$. Formally, let 
    \begin{align*}
        I_j &= \left[\frac{(1 +\delta)^j}{B}, \frac{(1 + \delta)^{j+1}}{B}\right),\\
        y_j &= \{x: w(x) \in I_j\}
    \end{align*}
    Clearly the number of sets in the partition is bounded by $m = O(\log(B)/\delta)$. 
    
    Since every $x \in y_j$ satisfies the condition $w(x) \in I_j$, for any $A \subset \X$ which intersects $y_j$, $w(A \cap y_j) \in I_j$. Also $w(y_j) \in I_j$. So it holds that 
    \[ \frac{w(A \cap y_j)}{w(y_j)} \in \left(\frac{1}{1 + \delta}, 1 + \delta\right).\]
\end{proof}

Note that the guarantee here is strong enough to recover a $(1 \pm \delta)$ multiplicative approximation to $w(A)$: we estimate the conditional probabilities $P(y_j|A) = P(y_j \cap A)/P(A)$ of the $y_j$s for the set $A$, and return the convex combination $\sum _{j \in [m]} P(y_j|A)w(y_j)$. Assuming for simplicity that the values $P(y_j|A)$ are correct, 
\begin{align*} 
    \sum _{j \in [m]} P(y_j|A)w(y_j) & \leq  \sum_{j \in [m]}\frac{P(y_j \cap A)}{P(A)}w(A \cap y_j) (1 + \delta) \\
    &= (1 + \delta)\sum_{j \in [m]} {P(y_j \cap A)}{P(A)}\frac{Q(A \cap y_j)}{P(A \cap y_j)}  \\
    &= (1 + \delta)\sum_{j \in [m]}\frac{Q(A \cap y_j)}{P(A)}\\
    &= (1 + \delta) \frac{Q(A)}{P(A)}
\end{align*}
Similarly one can show a lower bound of $(1 - \delta)w(A)$. 

But it is unclear how to estimate the values $w(x)$ for each point from random samples alone. Indeed, it is unclear how to even check if the statement $w(x) = w_0$ holds using random samples. 

We will form a partition $\Y = \{y_1, \ldots y_w\}$ of $\X$.


==> bounds.tex <==
\section{Sandwiching Bounds}


Given a weight function $w: \X \rgta \R$, what should the average weight  under $R$ of a point in $C$ be? 


We would like the following bounds to hold:
\begin{align}
\label{eq:sandwich}
    \E_{\x \sim P|_C}[w^*(\x)] \leq \E_{\x \sim R|_C}[w(\x)]  \leq \E_{\x \sim R|_C}[w^*(\x)].
\end{align}
We refer to these bounds as the {\em Sandwiching bounds}. 

Let us see why sandwiching bounds are natural desiderata for importance weights. The lower bound can be written as
\begin{align*}
    \E_{\x \sim P|_C}[w^*(\x)] = \frac{R(C)}{P(C)}.
\end{align*}
If this quantity is large, then the set $C$ is clearly anomalous on average, and we want our importance weights to reflect this. For instance, if a set is $10$ times more likely under $R$ than under $P$, we want the average anomaly score of a point sampled from $R|_C$ to be at least $10$. 

Of course, even if $R(C) = P(C)$ it is still possible that the set $C$ contains anomalies. But we want our scores to be conservative, they should not exaggerate the prevalence of anomalies within a set. This is why we require the bound
\[ \E_{\x \sim R|_C}[w(\x)]  \leq \E_{\x \sim R|_C}[w^*(\x)].\]


One can generalize this to anomaly scores of the form $g(w(x))$ where $g: \R \rgta \R$ is a univariate function such that $h(t) = t g(t)$ is convex. In particular, this includes $g(t) = \log(t)$ and $g(t) = t^\theta$ for $\theta \geq 0$. The case above where the scores are $w(x)$ corresponds to $g(t) = t$ and $h(t) = t^2$. 
For such functions, we will want our weights to satisfy
\begin{align}
\label{eq:g-sandwich}
    g\left(\E_{P|_C}[w^*(x)]\right) \leq \E_{R|_C}[g(w(x))]  \leq \E_{R|_C}[g(w^*(x))].
\end{align}
where the lower bound requires that sets that are clearly anomalous have high average scores, and the upper bound requires that the scores are conservative. Generalizing Equation \eqref{eq:sandwich2}, this is equivalent to  
\begin{align}
\label{eq:g-sandwich2}
    h\left(\E_{P|_C}[w^*(x)]\right) \leq \E_{P|_C}[w^*(x)g(w(x))]  \leq \E_{P|_C}[h(w^*(x))].
\end{align}


Note that if the distribution is $0$-multiAE, then 
\begin{align*}
    \E_{P|_C}[w(x)] = \frac{Q(C)}{P(C)} = \frac{R(C)}{P(C)} =  \E_{P|_C}[w^*(x)]
\end{align*}
One might expect that replacing $P|_C$ with $R|_C$ should only increase the expected value of $w(x)$, which would then imply the lower bound in Equation \eqref{eq:sandwich}. But somewhat surprisingly, we will see that this is not necessarily true. 



==> compare.tex <==
\section{Comparing Multiaccuracy and Multicalibration}\label{sec:compare}

In this section, we present examples highlighting the fact that the guarantees given by multicalibration are much stronger than what one obtains from multiaccuracy. We will use the setting of $\X = \zo^d$, with $\mC$ being the set of coordinate functions. Formally let $C_i^0 = \{x: x_i = 0\}$ and $C_i^1 = \{x: x_i = 1\}$ for all $i \in [d]$, and let $\mC = \{C^b_i\}_{i \in [d], b \in \zo}$. All our examples will use the following construction of multiaccurate distributions. 


The following Lemma stating that the maximum entropy distribution with a given set of marginal probabilities for $x_i$s is the product distribution is folklore. 
\begin{lemma}
    Let $P$ be the uniform distribution on $\zo^d$ and $R$ be an arbitrary distribution. Let $G^*$ denote the product distribution over $\zo^d$ such that $G^*(C^b_i) = R(C^b_i)$ for all $i \in [d]$. Then $G^*$ is the solution to Program \eqref{eq:prog1} for $\alpha =0$.
\end{lemma}
Let $\mS^*$ be the partition of $\zo^d$ based on weight. $G^*$ is the $(P,R, \mS^*)$-reweighted distribution over $\X$. Thus $\mS^*$ is $0$-multiaccurate. We will use $g(x) = G^*(x)/P(x)$ to denote importance weights of $Q^*$ with respect to $P$. 

If $w(x)$ corresponds to a $(0,0)$-mulitcalibrated partition, for any $S \in \mC$ by Equation \eqref{eq:exp-log-lb}
\[ \E_{\x \sim R|_S}[\log(w(x))] \geq \logf{R(S)}{P(S)} .\]
In  contrast we have the following claim.

\begin{lemma}
For any $\eta > 0$, there exists distributions $P, R$ and a $0$-multiaccurate partition $\mS^*$ such that the importance weights $g^*$ for the reweighted distribution satisfy
\begin{align*}
    \E_{\x \sim R|_S}[g^*(x)] \leq \frac{4\eta}{1 + 2\eta}\logf{R(S)}{P(S)}
\end{align*}
\end{lemma}
\begin{proof}
    Let $P$ be the uniform distribution on $\zo^2$. Let $R$ be given by
    \[ R(00) = 0, R(10) = R(01) = 1/2 -\eta, R(11) = 2\eta.\]
    The partition based on input weihgts is $0$-mulitcalibrated. 
    Then  $G^*$ is the product distribution where $\Pr[x_1 =1] = \Pr[x_2 =1] = 5/8$.
\end{proof}



We give an example shows that Equation \eqref{eq:exp-log-lb} does not hold under multiaccuracy. 


\begin{example}
\label{ex:1}
\end{example}

Let us consider the set $S = C_1^1$. We have $R(S) = 5/8$, $P(S) = 1/2$, hence $\log(R(S)/P(S)) = \log(5/4)$. Recall that by Equation \ref{eq:exp-log-lb}, this is a lower bound on the expected anomaly score under $R|_S$ for any mutlicalibrated distribution with $\alpha, \beta = 0$.
Wheres the expected anomaly scores under $R|_S$ are
\[E_{\x \sim R|_S}[\log(g^*(\x))] = \frac{3}{5}\logf{15}{16} + \frac{2}{5}\logf{25}{16} \leq \frac{4}{5}\logf{5}{4} = \frac{4}{5}\logf{R(S)}{P(S)}. \]
Generalizing this example, we can use $R(10) = R(01) = 1/2 - \eta$ and $R(11) = 2\eta$ to come up with an example where
\[ \E_{\x \sim R|_S}\log(g^*(x)) \leq \frac{4\eta}{1 + 2\eta} \logf{R(S)}{P(S)}.\]



==> consequences.tex <==
\section{Consequences of Multicalibration}\label{sec:consequences}



Given a partition $\mS$, every distribution $T$ over $\X$ naturally induces a distribution $T^\mS$ over $\mS$, where $\Pr_{\s \sim T^\mS}[\s = S] = T(S)$ for each $S \in \mS$.
For a partition $\mS$, let $\mFS$ denote the set of functions $f: \mS \rgta \R$. We can view these as functions $f: \X \rgta \R$ that are constant over set $S \in \mS$, and we will interchangeably use both views. An important example is the importance weight function $w$ of the $(P, R, \mS)$-weighted distribution $Q$. The following simple Lemma shows that any function in this class has identical expectations under $Q$ and $R$. Note that we do not assume that the partition is multicalibrated.

\begin{lemma}
    \label{lem:exp-equal}
    Let $\mS$ be  partition of $\X$ and let $Q$ be the $(P, R, \mS)$-reweighted distribution over $\X$. Then for any $f \in \mFS$, 
    \[ \E_{\x \sim R}[f(\x)] = \E_{\x \sim Q}[f(\x)].\] 
\end{lemma}
\begin{proof}
Note that for any function $f \in \mFS$ and any distribution $T$ over $\X$,
\begin{align}
    \label{eq:same-exp}
     \E_{\x \sim T}[f(\x)] = \sum_{x \in X}T(x)f(x) = \sum_{S \in \mS}f(S)\sum_{x \in S}T(x) = \sum_{S \in \mS}T(S)f(S) = \E_{\s \sim T^\mS}[f(\s)].
\end{align}
    Since $Q$ is the $(P, R, \mS)$- reweighted distribution over $\X$, $Q(S) =  R(S)$ for every $S \in \mS$ by definition, hence the induced distributions $Q^\mS$ and $R^\mS$ are  identical. So for $f \in \mFS$, it follows by Equation \eqref{eq:same-exp} that $\E_{\x \sim Q}[f(\x)] = \E_{\x \sim R}[f(\x)]$.
\end{proof}


 Our goal is to show that if $\mS$ is multicalibrated for $\mC$, then a similar claim holds after conditioning on any $C \in \mC$, that is,
$\E_{\x \sim Q|_C}[f(\x)]$ and $\E_{\x \sim R|_C}[f(\x)]$ are close to each other for all $f \in \mFS$. As a first step, we show that  multicalibration implies that the conditional distributions over the sets of the partition are close, that is, $Q|_C^\mS$ and $R|_C^\mS$ are statistically close.

\begin{lemma}
\label{lem:main}
Under Assumption \ref{asm:1}, for any $C \in \mC$,
    \[ \onenorm{Q|^\mS_C - R|^\mS_C} \leq   \frac{4\gamma}{R(C)}.\]
\end{lemma}
\begin{proof}
    Our approach is to use multicalibration to bound the contribution of each intersection of $C$ with the sets in $\mS$. Define $I \subseteq \{0, \ldots, m\}$ as $I = \{i: R|_C^\mS(S_i)  \geq Q|^\mS_C(S_i)\}$. We will bound the $L_1$ distance using
    \begin{align}
        \label{eq:u+v}
        \onenorm{Q|_C^\mS - R|^\mS_C} = 2\sum_{i \in I} R|_C^\mS(S_i) - Q|^\mS_C(S_i) = 2\sum_{i \in I} \frac{R(C \cap S_i)}{R(C)} - \frac{Q(C \cap S_i)}{Q(C)} .
    \end{align}
        
     If $0 \in I$, we can bound the contribution to \eqref{eq:u+v} from $S_0$ as
    \begin{align}
        \label{eq:from-u}
         \frac{R(C \cap S_0)}{R(C)} - \frac{Q(C \cap S_0)}{Q(C)} \leq \frac{R(C \cap S_0)}{R(C)} \leq \frac{\beta}{R(C)}.
    \end{align}
    The same bound also holds when $0 \not\in I$, since in this case the contribution to Equation \eqref{eq:u+v} is $0$. 
        
    We now bound the contribution from the rest of $I \setminus \{0\}$.  
    Since multicalibration implies multiaccuracy (Lemma \ref{lem:mc-ae}),
    \[ Q(C) \leq R(C) + \alpha + \beta. \]
    By definition multicalibration implies for each $i \in [m]$, 
    $Q(C \cap S_i) \geq R(C \cap S_i) -  \alpha R(S_i)$, so we have 
    \[ \frac{Q(C \cap S_i)}{Q(C)} \geq \frac{R(C \cap S_i) - \alpha R(S_i)}{R(C) + \alpha + \beta}.\]
    We can bound the contribution of $i$ to Equation \eqref{eq:u+v} by
    \begin{align*}
    \frac{R(C \cap S_i)}{R(C)} - \frac{Q(C \cap S_i)}{Q(C)} 
    \leq \frac{R(C \cap S_i)}{R(C)} - \frac{R(C \cap S_i) - \alpha R(S_i)}{R(C) + \alpha + \beta}
    = \frac{(\alpha + \beta)R(C \cap S_i) + \alpha R(C)R(S_i)}{R(C)(R(C) + \alpha + \beta)}.
    \end{align*}
    Summing over all $i \in [m]$, we get 
    \begin{align}
        \label{eq:from-v}
        \sum_{i \in [m]}  \frac{R(C \cap S_i)}{R(C)} - \frac{Q(C \cap S_i)}{Q(C)} &\leq \sum_{i \in [m]} \frac{(\alpha + \beta)R(C \cap S_i) + \alpha R(C)R(S_i)}{R(C)(R(C) + \alpha + \beta)}\notag\\
        & \leq \frac{(2\alpha + \beta)R(C)}{R(C)(R(C) + \alpha + \beta)} \leq \frac{2\alpha + \beta}{R(C)}.
    \end{align}
    Plugging Equations \eqref{eq:from-u} and \eqref{eq:from-v} into Equation \eqref{eq:u+v} gives the desired bound.
\end{proof}

We now show the following generalization of Lemma \ref{lem:exp-equal} under conditioning. 

\begin{theorem}
\label{thm:exp-bound}
Under Assumption \ref{asm:1}, for any $C \in \mC$ and $f \in \mFS$,  
    \[ \abs{\E_{\x \sim Q|_C}[f(x)]  - \E_{\x \sim R|_C}[f(x)]} \leq  \frac{4\gamma\infnorm{f}}{R(C)}.\]
\end{theorem}
\begin{proof}
By Equation \eqref{eq:same-exp},
\[ \E_{\x \sim Q|_C}[f(\x)] = \E_{\s \sim Q|_C^\mS}[f(\s)], \ \E_{\x \sim R|_C}[f(\x)] = \E_{\s \sim R|_C^\mS}[f(\s)]. \]
Hence
\begin{align*} 
\abs{\E_{\x \sim Q|_C}[f(x)]  - \E_{\x \sim R|_C}[f(x)]} &= \abs{\E_{\s \sim Q|^\mS_C}[f(\s)]  - \E_{\s \sim R|^\mS_C}[f(\s)]} \leq \onenorm{Q|_C^\mS - R|_C^\mS}\infnorm{f}. 
\end{align*}
The claim now follows from Lemma \ref{lem:main}.
\end{proof}


The above bound requires a bound on $\infnorm{f}$. We now show a bound on unnormalized expectations of functions in $\mFS$ that only requires boundedness of $f$ when $\beta > 0$. 

\begin{lemma}
\label{lem:omer}
    Let $C \in \mC$, let $f \in \mFS$. Under Assumption \ref{asm:1}
    \[ \abs{\sum_{x \in C} R(x)f(x)  - \sum_{x \in C} Q(x)f(x)} \leq \alpha \E_{\x \sim R}[|f(\x)|] + \beta \|f\|_\infty.\]
\end{lemma}
\begin{proof}
    Since $f \in \mFS$, we have
    \begin{align*}
        \sum_{x \in C} R(x)f(x) = \sum_{S \in \mS}f(S)\sum_{x \in C \cap S} R(x) = \sum_{S \in \mS} R(C \cap S)f(S),\\
        \sum_{x \in C} Q(x)f(x) = \sum_{S \in \mS}f(x)\sum_{x \in C \cap S} Q(x) = \sum_{S \in \mS}Q(C \cap S)f(S).
    \end{align*}
    Hence 
    \begin{align}
    \label{eq:sum-uv}
        \abs{\sum_{x \in C} R(x)f(x) - \sum_{x \in C} Q(x)f(x)} &= \abs{\sum_{i =0}^m (R(C \cap S_i) - Q(C \cap S_i)f(S_i)} \notag\\
        & \leq \sum_{i =0 }^m \abs{(R(C \cap S_i) - Q(C \cap S_i))f(S_i)}. 
    \end{align}
    Using Equation \eqref{eq:add-beta}, we have
    \begin{align}
    \label{eq:bound-0}
        \abs{(R(C \cap S_0) - Q(C \cap S_0))f(S_0)} & \leq \beta \|f\|_\infty.
    \end{align}
    For the other $S_i$s, using the definition of multicalibration,
    \begin{align}
    \label{eq:bound-m}
        \sum_{i=1}^m \abs{R(C \cap S_i) - Q(C \cap S_i))f(S_i)} & \leq  \sum_{i=1}^m\alpha R(S_i)|f(S_i)| \leq  \alpha\E_{\x \sim R}[|f(x)|]    .
    \end{align}
    Plugging Equations \eqref{eq:bound-0} and \eqref{eq:bound-m} into Equation \eqref{eq:sum-uv} proves the claim.
\end{proof}










\eat{
\subsection{Multicalibrated Partitions}
In order to construct multicalibrated weight functions, we will focus on a special family of functions that arise naturally from partitions. 

\begin{definition}
    Let $\mS = \{S_1, \ldots, S_m\}$ be a partition of $\X$. The canonical weight function $w$ for this partition is
    \[ w(x) = \frac{R(S_i)}{P(S_i)} \ \text{if} \ x \in S_i \ \text{for}\ i \in [m]. \]
    The canonical distribution $Q$ is given by
    \[ Q(x) = w(x)P(x) = \frac{P(x)R(S_i)}{P(S_i)} = R(S_i)P(x|S_i).\]
    We say that the partition is $\alpha$-multicalibrated if $w$ is $\alpha$-multicalibrated.
\end{definition}

For simplicity, we will assume that the partition is minimal meaning that $w(S_i) \neq w(S_j)$ for $i \neq j$. We can ensure minimality by merging $S_i, S_j$ which violate this condition. 
It is easy to see that the canonical distribution $Q$ and $R$ give equal weight to each $S_i \in S$ (hence $Q$ is $0$-multi-AE for $\mS$ under $R$. More generally we have the following bound.

\begin{lemma}
\label{lem:eq-wt}
    For $Q$ as above, $i \in [m]$, and $B \subseteq S_i$,
    \begin{align}
        Q(B)  = R(S_i)\frac{P(B)}{P(S_i)}.
    \end{align}
    In particular $Q(S_i) = R(S_i)$ for $i \in [m]$. 
\end{lemma}
\begin{proof}
For $B \subseteq \S_i$, we have 
\[ Q(B) =  \sum_{x \in B} w(x)P(x)=  \frac{R(S_i)}{P(S_i)}\sum_{x \in B}P(x) = R(S_i)\frac{P(B)}{P(S_i)}. \]
\end{proof}


We now apply Theorem \ref{thm:omer} 

\begin{lemma}
Let $w$ be the canonical weight function of the partition $\mS = \{S_1, \ldots, S_m\}$. Let $B = max_{i \in [m]}R(S_i)/P(S_i)$. Then
\begin{align}
    \abs{\sum_{x \in C} R(C \cap S_i)\logf{R(S_i)}{P(S_i)}  - \KL{Q(x|C)}{P(x|C)}} \leq \alpha \KL{R(x)}{P(x)} + (1 + \alpha)\beta \log(B).
\end{align}
\end{lemma}

For weight functions arising from partitions, the definition of multicalibration can be restated purely in terms of properties of the partition as follows. 

\begin{lemma}
\label{lem:restate}
Let $\alpha >0$, let $\mC \subseteq 2^\X$ be a collection of sets, and let $\mS = \{S_1, \ldots, S_m\}$ be a partition of $\X$. $\mS$ is $\alpha$-multicalibrated for $\mC \subseteq 2^\X$ under $R$ if for every $C \in \mC, i \in [m]$
    \begin{align}
        \label{eq:big2} 
        \abs{\frac{P(C \cap S_i)}{P(S_i)}  - \frac{R(C \cap S_i)}{R(S_i)}} & \leq \alpha.
    \end{align}
\end{lemma}
\begin{proof}
By minimality, each set $S_v$ corresponds to a unique $S_i \in \mS$, so we relabel the states $\{S_v\}_{v \in W}$ as $S_1, \ldots, S_m$ for $m = |W|$. Equation \eqref{eq:big} requires that for all $C \in \mC, i \in [m]$, 
    \begin{align} 
        \label{eq:eq2r}
        \abs{Q(C \cap S_i)  - R(C \cap S_i)} & \leq \alpha R(S_i). 
    \end{align}
    Note that 
    \[ Q(C \cap S_i) = \sum_{x \in C \cap S_i} P(x)\frac{R(S_i)}{P(S_i)} =  \frac{P(C \cap S_i) R(S_i)}{P(S_i)}. \] 
Plugging this into Equation \eqref{eq:eq2r} and dividing by $R(S_i)$ gives Equation \eqref{eq:big2}.
\end{proof}
}


\eat{
Since $S = h^{-1}(b)$, for every $y \in \Y$
\begin{align*}
    \eps_y = \left| \E_{x \sim r(x|y)}[h(x)] - \E_{x \sim p(x|y)}[h(x)]\right| = \lst r(S|y)  - p(S|y)\rst, \\
    \lst q(S) - r(S)\rst =  \abs{\sum_y r(y)r(S|y) - \sum_y r(y)p(S|y)} \leq \sum_yr(y)\eps_y \leq \eps.
\end{align*} 
Hence
    \[ q_S(y)  = \frac{r(y)p(S|y)}{q(S)} \geq \frac{r(y)(r(S|y) - \eps_y)}{r(S) + \eps} = \frac{r(y \cap S) - \eps_y r(y)}{r(S) + \eps}.\]
We use this to bound the distance between $r_S(y)$ and $p_S(y)$ as follows:
\begin{align*}
    \norm{r_S(y) - q_S(y)} & = 2 \sum_{y: r_S(y) > q_S(y)}r_S(y) - q_S(y) \\
    & \leq 2\sum_{y} \frac{r(y \cap S)}{r(S)} - \frac{r(y \cap S) - \eps_y r(y)}{r(S) + \eps}\\
    &= 2\frac{\sum_y\eps r(y \cap S) + \sum_y\eps_y r(y)r(S)}{r(S)(r(S) + \eps)}\\
    & \leq\frac{4\eps}{r(S) + \eps}
\end{align*}
where we use $\sum_y r(y \cap S) = r(S)$ and $\sum_y\eps_yr(y) \leq \eps$.
}

==> old_stuff/anomalous.tex <==
\section{Finding Anomalous Sets}

For a given class of hypothesis/sets $\mathcal{F}$, consider all possible ``intersections'' of the sets $f\in \mathcal{F}$. Let this be the set $\mathcal{S}$. Let the distribution $q$ be indistinguishable from $r$ with respect to $S$ and be max-entropy with respect to $p$. We want to then show that
\begin{align}
    \sum_{x\in f}  r(x) \log \frac{q(x)}{p(x)} \ge  r(f)\log \frac{r(f)}{p(f)}.
\end{align}
By the log-sum inequality,
\begin{align}
    \sum_{s: s \subseteq f, s\in \mathcal{S}}  r(s) \log \frac{r(s)}{p(s)} \ge  r(f)\log \frac{r(f)}{p(f)}. \label{eq:log_sum1}
\end{align}
We claim that for any $s\in \mathcal{S}$
\begin{align}
    \frac{r(s)}{p(s)}=\frac{q(s)}{p(s)}=\frac{q(x)}{p(x)}, \text{ where } x \in s.\label{eq:max_ent}
\end{align}
Plugging this into \eqref{eq:log_sum1} yields the desired relationship,
\begin{align}
      r(f)\log \frac{r(f)}{p(f)} &\le  \sum_{s: s \subseteq f}  r(s) \log \frac{r(s)}{p(s)} \\
      &= \sum_{s: s \subseteq f}  r(s) \log \frac{q(s)}{p(s)} \\
      &= \sum_{s: s \subseteq f} \sum_{x: x\in s}  r(x) \log \frac{q(x)}{p(x)}\\
      &= \sum_{x\in f}  r(x) \log \frac{q(x)}{p(x)}.
\end{align}
We now verify \eqref{eq:max_ent}. Note that $f_i(x)$ is constant for all $i$ for all $x\in s$. Therefore since $q$ is max-entropy with respect to $p$,
\begin{align}
    q(x) &= p(x) \exp(\sum_i \lambda_i f_i(x)-\lambda_0),\\
    \implies  \sum_{s\in s} q(x) &=  \exp(\sum_i \lambda_if_i(x)-\lambda_0)\sum_{s\in s}  p(x)\\
    \implies \frac{q(s)}{p(s)}&=\frac{q(x)}{p(x)}=\exp(\sum_i \lambda_i f_i(x)-\lambda_0).
\end{align}
Since $q$ and $r$ are indistinguishable with respect to $\mathcal{S}$, for any $s\in \mathcal{S}$,
\begin{align}
   \frac{q(s)}{p(s)}=\frac{r(s)}{p(s)},
\end{align}
which verifies \eqref{eq:max_ent}.

An additional inequality that might be useful. Suppose $q$ is not max-entropy with respect to $\mathcal{S}$, which is exponentially larger than $\mathcal{F}$. 

\begin{lemma}
    We have 
    \begin{align}
        \sum_{x\in f}  \frac{r(x)}{r(f)} \log \frac{q(x)}{p(x)} \geq \log\left(\frac{r(f)}{p(f)}\right) -  \log\left(\sum_{x \in f}\frac{p(x)r(x)}{p(f)q(x)}\right) 
    \end{align}
\end{lemma}
\begin{proof}
Consider the random variable $Y$ which takes the value $p(x)/q(x)$ with probability $r(x)/r(f)$ over $x \in f$, so that 
\begin{align}
    \E[Y] &= \sum_{x \in f} \frac{p(x)}{q(x)}\frac{r(x)}{r(f)}\\
        &= \frac{p(f)}{r(f)} \sum_{x\in f}\frac{p(x)r(x)}{p(f)q(x)}
\end{align}
Now consider the convex function $\log(1/y)$. By Jensen's inequality,
\begin{align}
  \sum_{x \in f}\frac{r(x)}{r(f)}\log\left(\frac{q(x)}{p(x)}\right) &= \E[\log(1/Y)] \geq \log\left(\frac{1}{E[Y]}\right)\\
  &= \log\left(\frac{r(f)}{p(f)}\right) - \log\left(\sum_{x \in f} \frac{p(x)r(x)}{p(f)q(x)} \right)
\end{align}
which proves the claim.
\end{proof}
Since
\[ \frac{p(x)r(x)}{p(f)q(x)} = \E_{p|_f}\left[\frac{r(x)}{q(x)}\right] \]
this tells us that if expected ratio of $r/q$ under $p$ conditioned on $f$ is small, then the average anomaly score over $f$ gets close to $\log(r(f)/p(f))$. 
}


==> old_stuff/pinsker.tex <==
\section{A Reverse Pinsker Inequality}

Define the $\ell_1$ distance between two distributions $r, p$ on the same discrete domain $\Y$ as
    \[ \| r - p\|_1 = \sum_{y \in \Y}|r(y) - p(y)|. \]
Pinkser's inequality states that
\[ \KL{r}{p} \geq \frac{1}{2\log(2)}\|r - p\|_1^2 .\]
We will show a "reverse" Pinsker inequality, that the KL divergence $\KL{r}{p}$ can be bounded, provided that the $\ell_1$ distance is bounded, and the ratio $r(y)/p(y)$ is not too large. The example of Bernoulli random variables with parameters $p =0$ and $r = \eps$ shows that when $\|r - p\|_1 \leq \eps$, the KL divergence can be unbounded, so some extra assumption is needed. 

\begin{theorem}
\label{thm:rev-pinsker}
Let $r$ and $p$ be two distributions over a domain $\Y$, such that 
\begin{align}
    \frac{r(x)}{p(x)} &\leq B \ \ \forall x \in \X.
\end{align} 
Then
\begin{align}
    \KL{r}{p} \leq \|r - p\|_1\frac{ B\log(B)}{2(B -1)}.
\end{align}
Indeed for any $S \subseteq \Y$,
\begin{align}
    \sum_{y \in S}r(y)\logf{r(y)}{p(y)} \leq \|r - p\|_1\frac{ B\log(B)}{2(B -1)}.
\end{align}
\end{theorem}


Let 
\begin{align*}
    S^+ = \{y: r(y) > p(y)\}, \ S^0 = \{y: r(y)  =p(y)\}, S^- = \{y: r(y) < p(y)\}
\end{align*}
Assuming $r$ and $p$ are not identical, $S^+$ and $S^-$ are non-empty, and further
\[ \sum_{y \in S^+}r(y) - p(y) = \sum_{y \in S^-} p(y) - r(y)  = \frac{1}{2}\|r -p \|_1 .\]
Note that $\logf{r(y)}{p(y)}$ is positive on $S^+$, negative on $S^-$ and $0$ on $S^0$. Hence, the sum 
$\sum_{y \in S}r(y)\logf{r(y)}{p(y)}$ is maximized for $S = S^+$, and
\begin{align}
    \label{eq:s+-}
    \KL{r(y)}{p(y)} = \sum_{y \in S^+}r(y)\logf{r(y)}{p(y)} - \left| \sum_{y \in S^-}r(y)\logf{r(y)}{p(y)} \right| \leq \sum_{y \in S^+}r(y)\logf{r(y)}{p(y)}. 
\end{align} 
Hence Theorem \ref{thm:rev-pinsker} is implied by the following lemma.

\begin{lemma}
\label{lem:s+}
We have
\begin{align}
    \label{eq:s+}
    \sum_{y \in S^+} r(y) \logf{r(y)}{p(y)} \leq \|r - p\|_1 \frac{B\log(B)}{2(B -1)}.
\end{align}
\end{lemma}
\begin{proof}
Hence, in order to prove the claim for arbitrary $S \subseteq \X$, it suffices to show it for $S^+$.
    For each point $y \in S^+$, let  
    \begin{align*}
            r(y) - p(y) = \eps_y \geq 0,\\
            \frac{r(y)}{p(y)} = B_y \in (1, B].
    \end{align*}
    Then we can write
    \begin{align*}
        r(y) &= \eps_y\frac{B_y}{B_y -1},\\
        p(y) &= \eps_y \frac{1}{B_y -1}\\
        r(y)\logf{r(y)}{p(y)} &= \eps_y  \frac{B_y\log(B_y)}{B_y -1} \leq \eps_y \frac{B\log(B)}{B-1}
    \end{align*}
    where the last inequality hold because the function $h(x) = x \log(x)/(x-1)$ is increasing for $x \geq 1$.   Since $\sum_{y\ in S^+} \eps_y = \|r - p\|_1$, we have
    \[\sum_{y \in S} r(y) \logf{r(y)}{p(y)} \leq \frac{B\log(B)}{B-1}\sum_{y \in \Y} \eps_y  \leq \|r - p\|_1\frac{B \log(B)}{2(B-1)}.\]
\end{proof}

Next we will show the following bound on the sum of the absolute values of $\log(r(y)/p(y))$.
\begin{corollary}
\label{thm:abs-val}
Let $r$ and $p$ be two distributions over a domain $\Y$, such that 
\begin{align}
    \frac{r(x)}{p(x)} &\leq B \ \ \forall x \in \X. 
\end{align} 
Then
\begin{align}
    \label{eq:abs-val}
    \sum_{y \in \Y}r(y)\left|\logf{r(y)}{p(y)}\right| \leq \|r - p\|_1\frac{ B\log(B)}{(B -1)}.
\end{align}
\end{corollary}
\begin{proof}
Grouping terms by their sign and ignoring the $0$ terms, 
\begin{align}
    \label{eq:abs-val2}
    \sum_{y \in \Y}r(y)\left|\logf{r(y)}{p(y)}\right| = \sum_{y \in S^+}r(y)\logf{r(y)}{p(y)} + \left|\sum_{y \in S^-}r(y)\logf{r(y)}{p(y)}\right| 
\end{align}
Note that 
\[\KL{r(y)}{p(y)} = \sum_{y \in S^+} r(y) \logf{r(y)}{p(y)} - \left|\sum_{y \in S^-} r(y) \logf{r(y)}{p(y)}\right| \geq 0. \]
By Lemma \ref{lem:s+}, this implies that 
\[ \left|\sum_{y \in S^-} r(y) \logf{r(y)}{p(y)}\right| \leq \sum_{y \in S^+} r(y) \logf{r(y)}{p(y)} \leq 
\|r - p\|_1 \frac{B\log(B)}{2(B -1)} \]
Plugging this into Equation \eqref{eq:abs-val2}, along with the bound from Equation \eqref{eq:s+} for the positive part implies the claim.
\end{proof}

In fact one can remove the dependence on $B$ altogether for the $S^-$ part, although this will not change the asymptotic bound in Equation \eqref{eq:abs-val}.

\begin{lemma}
\label{lem:s-}
We have 
\begin{align}
    \left|\sum_{y \in S^-} r(y) \logf{r(y)}{p(y)}\right| \leq  \frac{\|r - p\|_1}{2}.
\end{align}
\end{lemma}
\begin{proof}

Consider the univariate function $g:[0,1 - \eps] \rgta \R$ defined as
\[ g(r) = r\logf{r}{r + \eps}. \]
Simple calculus shows that this is a decreasing function of $r$, hence it is minimized at $r = 1 - \eps$, where it takes the value
\[ g(1 - \eps) = (1 - \eps)\log(1 - \eps) \geq -\eps(1 - \eps) \geq -\eps.\]

Let $\eps = \|r - p\|_1/2$, so that $p(S^-) = r(S^-) + \eps$. By the log-sum inequality,
\begin{align*} 
    \sum_{y \in S^-} r(y) \logf{r(y)}{p(y)} &\geq \left(\sum_{y \in S^-} r(y)\right)\frac{\left(\sum_{y \in S^-} r(y)\right)}{\left(\sum_{y \in S^-} p(y)\right)} \\
    &= r(S^-)\logf{r(S^-)}{r(S^-) + \eps} \geq -\eps
\end{align*}
which implies the claim by taking absolute values. 
\end{proof}



==> old_stuff/pythagoras.tex <==
\section{Guarantees}

For $S \subset \X$ and a distribution $r$ on $\X$, let $r_S$ denote the distribution $r$ conditioned on $S$, so that $r_S(x) = r(x)/r(S)$ for all $x \in S$.

Upon termination, we will show that for every set $S =h^{-1}(b)$ where $b \in \zo$, the following approximate Pythagorean theorem holds:

\begin{align*}
    \left|\KL{r_S}{p_S} - \KL{r_S}{q_S} - \KL{q_S}{p_S}\right| \leq \eps \log(B).
\end{align*}

We have
\begin{align*}
    \KL{r_S}{p_S} -\KL{r_S}{q_S}  &= \sum_{x \in S}r_S(x)\logf{q_S(x)}{p_S(x)}\\ 
    &= \sum_{x \in S}\frac{r(x)}{r(S)}\logf{q(x)p(S)}{p(x)r(S)}\\
    &= \sum_{x \in S}\frac{r(x)}{r(S)}\logf{q(x)}{p(x)} + \logf{p(S)}{r(S)}\\
\end{align*}
Recall that $q(x) = r(y)p(x|y)$. Hence $q(x)/p(x) = r(y)/p(y)$.
\begin{align*}
    \KL{r_S}{p_S} -\KL{r_S}{q_S}  = \sum_{x \in S}\frac{r(x)}{r(S)}\logf{q(y)}{p(y)} = \sum_{y \in \Y}\frac{r(y \cap S)}{r(S)}\logf{q(y)}{p(y)}
\end{align*}

On the other hand
\begin{align*}
    \KL{q_S}{p_S} &= \sum_{x \in S}\frac{q(x)}{q(S)}\logf{q(x)p(S)}{p(x)q(S)}\\
    &= \sum_{x \in S}\frac{q(x)}{q(S)}\logf{q(x)}{p(x)} + \logf{p(S)}{q(S)}\\
    & = \sum_{y \in \Y}\frac{q(y \cap S)}{q(S)}\logf{r(y)}{p(y)} + \logf{p(S)}{q(S)}
\end{align*}
Hence we can write 
\begin{align*}
    \KL{r_S}{p_S} - \KL{r_S}{q_S} - \KL{q_S}{p_S} = \sum_{y \in \Y}\left(\frac{r(y \cap S)}{r(S)} - \frac{q(y \cap S)}{q(S)}\right)\logf{r(y)}{p(y)} + \logf{q(S)}{r(S)}
\end{align*}
We now relate $r(y \cap S)$ and $q(y \cap S)$. We have
\begin{align*} 
    \frac{r(y \cap S)}{r(S)} = \frac{r(y)r(S|y)}{r(S)},\\ 
    \frac{q(y \cap S)}{q(S)} = \frac{r(y)p(S|y)}{q(S)}. 
\end{align*}
Note that $|r(S|y) - p(S|y)| = \eps_y$, and $|r(S) - p(S)| = \E_{r}[\eps_y]$. Hence 
\begin{align*} 
    \left|\frac{r(y \cap S)}{r(S)} -    \frac{q(y \cap S)}{q(S)} \right| \leq  . 
\end{align*}




==> prelims-impweights.tex <==
\section{Preliminaries}

We use capitals $(P, Q, R, \cdots)$ to denote distributions and boldface $\x, \y, \cdots$ to denote random variables. We use $\x \sim P$ to denote sampling the variable $\x$ according to distribution $P$, and $\x \sim P_A$ to denote sampling from $P$ conditioned on an event $A \subseteq \X$, so that $P_A(x) = P(x)/P(A)$. We use $Q \ll P$ to denote that the support of $Q$ is contained in that of $P$. We use $\log$ to denote logarithms to base $2$ and $\ln$ for natural logarithms. 

To every distribution $Q(x)$, one can associate a function $w(x) = Q(x)/P(x)$, which we call the (importance) weight function of $Q$ relative to $P$. Any function $w: \X \rgta \R^+$ which satisfies $\E_{\x \sim P}[w(\x)]  = 1$ can be used to define a distribution $Q$ as $Q(x) = w(x)P(x)$. We refer to such functions as weight functions for short.  We will often consider the conditional expectations of weight functions. 

\begin{lemma}
\label{lem:cond-ex}
    For any subset $C \subseteq \X$,
    \[ \E_{\x \sim P_{C}}[ w(x)] = \frac{Q(C)}{P(C)}\]
\end{lemma}
\begin{proof}
    \[  Q(C) = \sum_{x \in C} Q(x) =  \sum_{x \in C} w(x)P(x) = P(C)  \sum_{x \in C} w(x)\frac{P(x)}{P(C)} = P(C) \E_{\x \sim P_C} [w(x)].\]
\end{proof}


Given a prior distribution $P$ and the observed distribution $R$, let us denote the importance weights of $R$ relative to $P$  as $w^*(x) = R(x)/P(x)$. Say we are trying to build a model $Q$ for $R$ by assigning importance weights $w:\X \rgta \R$. 
Every set $C \subseteq \X$ defines a statistical test where we take random samples according to a distribution $Q$ and measure the fraction $Q(C)$ that lie in $S$. We say $w$ is accurate in expectation if $Q$ is near indistinguishable from $R$ under this test.

\begin{definition}
\label{def:ae}
    Let $\alpha >0$, let $\mC \subseteq 2^\X$ be a collection of sets. Let $w:\X \rgta \R$ be the weight function of $Q$ relative to $R$. The weight function $w$ is $\alpha$-multi-accurate in expectation ($\alpha$-multiAE) for $\mC \subseteq 2^\X$ under $R$ if for every $C \in \C$, it holds that
    \begin{equation}
        \label{eq:def-ae}
        |Q(C)  - R(C)| \leq \alpha.
    \end{equation}  
      
\end{definition}

Equivalently, by Lemma \ref{lem:cond-ex} w is $\alpha$-multiAE for $\mC$ under $R$ if for every $C \in \mC$,
    \[ \abs{ \E_{\x \sim P_C}[( w(x) -  w^*(x))] }\leq \frac{\alpha}{P(C)}.\]

\eat{
The following Lemma connects our definition to the notion of accuracy in expectation as defined in the supervised setting. 

\begin{lemma}
\label{lem:equiv-def}
    The weight function $w$ is $\alpha$-AE for $C$ under $R$ iff
    {lemma}
\begin{proof}
    We have 
    \[ P(C)\E_{\x \sim P_{|C}}[w(x)] =  Q(C), \ \  P(C) \E_{\x \sim P_{|C}}[w(x)] =  R(C).\]
    Hence 
    \[ \abs{\E_{\x \sim P_{|C}}[w(x)] - \E_{\x \sim P_{|C}}[w^*(x)]} =  \frac{\left|Q(C) - R(C)\right|}{P(C)}\]
    from which the proof follows.
\end{proof}
}

Next we introduce the stronger notion of multicalibration. It will be convenient to restrict the weight function $w$ to only take on finitely many distinct values. So we assume $w:\X \rgta V \subset \R^+$. For $v \in V$, let $S_v = \{x \in \X: w(x) = v \}$ so that $\{S_v\}_{v \in W}$ is a partition of $\X$. 

\begin{definition}
    \label{def:a-multic}
    ($\alpha$- multicalibration) 
    Let $\alpha >0$, let $\mC \subseteq 2^\X$ be a collection of sets. Let $w:\X \rgta V$ be the weight function of $Q$ relative to $R$. The weight function $w$ is $\alpha$-mulitcalibrated for $\mC \subseteq 2^\X$ under $R$ if for every $C \in \mC$ and $v \in V$, it holds that
    \begin{align}
        \label{eq:big} \abs{Q(C \cap S_v)  - R(C \cap S_v)} & \leq \alpha R(S_v)
    \end{align}
\end{definition}
Multicalibration is a stronger guarantee than multi-accuracy in expectation. This follows easily by summing Equation \eqref{eq:big} over all $v \in V$. 
For each  weight $v \in V$ and $C \in \mC$, $\alpha$-calibration requires that
\[ Q(C \cap S_v) = R(C \cap S_v) \pm \alpha R(S_v) .\]
If $R(C \cap S_v)/R(S_v)$ is not too small, this translates to a multiplicative guarantee for $Q(C \cap S_v)$. We can restate this condition in terms of importance weights following Lemma \ref{lem:cond-ex}, along with the observation that $w(x) = v$ for all $x \in S_v$.  
\begin{corollary}
    If the weight function $w$ is $\alpha$-calibrated for $C$ under $R$ then for each $v \in V$
    \[ \abs{ \E_{\x \sim P_{S_v}}[ w^*(x)] -  v }\leq \frac{\alpha R(S_v)}{P(C \cap S_v)}.\]
\end{corollary}


The requirement in Equation \eqref{eq:big} can be hard to satisfy efficiently for sets $S_v$ such that $R(S_v)$ is very small; this motivates a relaxed notion that we call $(\alpha, \beta)$-multicalibration. 

\begin{definition}
\label{def:ab-multic}    
Let $\alpha >0, \beta > 0$, let $\mC \subseteq 2^\X$ be a collection of sets. Let $w:\X \rgta \R$ be the weight function of $Q$ relative to $R$. The weight function $w:\R \rgta W$ is $(\alpha, \beta)$-multicalibrated for $\mC \subseteq 2^\X$ under $R$ if we can partition the range $W$ into disjoint sets $U, V$ such that 
\begin{align}
\label{eq:small}
\sum_{u \in U}(Q(S_u)  + R(S_u)) \leq \beta,
\end{align}
and for every $C \in \mC$ and $v \in V$, it holds that
    \begin{align}
        \label{eq:big2} 
        \abs{Q(C \cap S_v)  - R(C \cap S_v)} & \leq \alpha R(S_v)
    \end{align}
\end{definition}

The case $\beta = 0$ corresponds to $\alpha$-multicalibration. $(\alpha, \beta)$-multicalibration permits a {\em bad} subset $\X_U = \cup_{u \in U} S_u$ that does not satisfy Equation \eqref{eq:big2}, but this subset has small measure under both $Q$ and $R$.

\begin{lemma}
\label{lem:mc-ae}
    If $w$ is $(\alpha, \beta)$-multicalibrated for $\mC$ under $R$, then  it is $(\alpha + \beta)$-AE for $\mC$ under $R$.
\end{lemma}
\begin{proof}
    We bound the contributions from $U$ and $V$ separately. By Equation \eqref{eq:big2}, 
    \begin{align*}
        \sum_{v \in V} \abs{Q(C \cap S_v)  - R(C \cap S_v)} \leq \sum_{v \in V} \alpha R(S_v) \leq \alpha,
    \end{align*} 
    To bound the contribution from $U$, we use Equation \eqref{eq:small}:
    \begin{align*}
        \sum_{u \in U} |Q(C \cap S_u)  - R(C \cap S_u)| \leq \sum_{u \in U} (R(S_u)  + Q(S_u))  \leq \beta. 
    \end{align*}
    The claim follows since
    \begin{align*}
        \abs{Q(C) - R(C)} \leq \sum_{v \in V} \abs{Q(C \cap S_v)  - R(C \cap S_v)} + \sum_{u \in U} \abs{Q(C \cap S_u)  - R(C \cap S_u)}.
    \end{align*}
\end{proof}




\eat{
We now state the stronger notion of multi-calibration, which requires simultaneous calibration over all tests $C \in \mC$. 

\begin{definition}
    \label{def:multi-c}
    ($\alpha$-multicalibration)
    Let $\alpha, \beta \geq 0$ and $\mC \subseteq 2^\X$. The weight function $w$ is $(\alpha, \beta)$-multicalibrated for $\mC$ under $R$ if there exists $V \subseteq W$ such that 
\begin{align}
    \label{eq:big}\forall C \in \mC, \forall v \in V,\ \abs{Q(C \cap S_v)  - R(C \cap S_v)} & \leq \alpha R(S_v),\\
    \label{eq:small} \sum_{v \not\in V} (Q(S_v) + R(S_v)) & \leq \beta
    \end{align}
\end{definition}


Similarly, we can define the weaker notion of multi-accuracy in expectation (multi-AE). 
\begin{definition}
    ($\alpha$-multi-AE)
    For $\alpha > 0$ and $\mC \subseteq 2^\X$, the weight function $w$ is $\alpha$ multi-accurate in expectation ($\alpha$-multi-AE) for $\C$ under $R$ if it is $\alpha$-AE for every   $C \in \mC$.
\end{definition}

Since multicalibration implies that every $C \in \mC$ is calibrated, and $(\alpha, \beta)$-calibration implies $(\alpha+ \beta)$-AE, it follows that $(\alpha, \beta)$-multicalibration for $\mC$ under $R$ implies $(\alpha + \beta)$-multi-AE for $\mC$ under $R$.  





\subsection{Multicalibrated Partitions}

Having defined multicalibration for general (discrete) weight functions, we will focus on a particular family of functions that arise naturally from partitions of $\X$. 
We have seen that every discrete weight function $w: \X \rgta \W$ induces a partition $\{S_v\}_{v \in W}$ of $\X$. Conversely, one can associate a weight function to any partition as follows.


We have 
\[  \E_{\x \sim P}[w_\ms(x)] = \sum_{x \in \X}  P(x)\fraC{R(S_i)}{P(S_i)} = \sum_{i \in [m]}P(S_i)\frac{R(S_i)}{P(S_i)} = 1\] 
so $w_\mS$ is a valid weight function. Since 
\[ Q_\mS(S_i) =  \sum_{x \in S_i} w_\mS(x)P(x)=  \frac{R(S_i)}{P(S_i)}\sum_{x \in S_i}      P(x) = R(S_i), \] 
it follows that $w_\mS$ is $0$-multi-AE for $\mS$ under $R$.  Further, 
\[ Q_\mS(x) = w_\mS(x)P(x) = \frac{R(S_i)}{P(S_i)}P(x) = R(S_i)P_{|S_i}(x),\] 
so $Q_\mS$ can be interpreted as first sampling a partition $S_i \in \mS$ according to $R$ and then sampling $x \in S_i$ according to $P_{|S_i}$. 



\begin{lemma}
    Given a partition $\mS$, the associated weight function $w_\mS$ is $(\alpha, \beta)$-multicalibrated for $\mC$ under $R$ iff
    there exists $I \subseteq [m]$ such that 
    \begin{align}
        \label{eq:big2}\forall C \in \mC, \forall i \in I,\ \abs{\frac{P(C \cap S_i)}{P(S_i)}  - \frac{R(C \cap S_i)}{R(S_i)}} & \leq \alpha ,\\
        \label{eq:small2} \sum_{i \not\in I} R(S_i) & \leq \beta/2
    \end{align}
\end{lemma}
\begin{proof}
    We will show that these conditions are essentially a restatement of those in Definition \ref{def:multi-c}. Since $w_\mS$ is constant on each $S_i$ and distinct across $S_i$s, the set of values $V \subseteq W$ corresponds to a set of indices $I = \{i \subseteq [m]: w(S_i) \in V\}$. 
    
    Fix $i \in I$. Equation \eqref{eq:big} is equivalent to saying that for all $C \in \mC, i \in I$, 
    \[ \abs{Q(C \cap S_i)  - R(C \cap S_i)} & \leq \alpha R(S_i). \]
    Dividing by $R(S_i)$ gives Equation \eqref{eq:big2}.
    
    For any $i \in [m]$, $Q(S_i) = R(S_i)$. Hence we can rewrite \eqref{eq:small} as \eqref{eq:small2}.
\end{proof}

}

==> pythagoras.tex <==
\section{An Approximate Pythagorean Theorem for Multicalibrated Partitions}
\label{sec:pythagorean}

If $Q$ is the $(P, R, \mS)$ reweighted distribution over $\X$, then the following {\em Pythagorean} theorem holds for the distributions $P, Q$ and $R$.  It can be viewed as a consequence of the chain rule for KL divergence for the pair of variables $(x, S)$ where $x \in S$.  Note that we do not assume multicalibration for this statement. 


\begin{lemma}
\label{lem:pyth}
    Let $\mS$ be  partition of $\X$ and let $Q$ be the $(P, R, \mS)$-reweighted distribution over $\X$. Then
    \begin{equation}
        \nonumber
        \KL{R}{P} - \KL{R}{Q} = \KL{Q}{P}.
    \end{equation}
\end{lemma}
\begin{proof}
    We can write the LHS as
    \begin{align*}
        \KL{R}{P} - \KL{R}{Q} = \sum_{x \in \X}R(x)\logf{Q(x)}{P(x)} = \sum_{S \in \mS} \sum_{x \in S} R(x)\logf{R(S)}{P(S)} = \sum_{S \in \mS}  R(S)\logf{R(S)}{P(S)}
    \end{align*}
    where the second equality is by the definition of $Q$.
    We can write the RHS as
    \begin{align*}
        \KL{Q}{P} = \sum_{x \in \X} Q(x)\logf{Q(x)}{P(x)} = \sum_{S \in \mS} Q(S)\logf{R(S)}{P(S)} = \sum_{S \in \mS}  R(S)\logf{R(S)}{P(S)}
    \end{align*}
    where the first equality if by the definition of $Q$ and the second since $Q(S) = R(S)$.
\end{proof}


If we assume multicalibration, for every $C \in \mC$, we get an approximate Pythagorean theorem for the conditional distributions $R|_C$, $P|_C$ and $Q|_C$. 

\begin{theorem}
\label{thm:pyth1}
Under Assumption \ref{asm:1} and the $B$-boundedness assumption, for any $C \in \mC$ we have
\begin{align}
    \label{eq:p-simple2}
    \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \KL{Q|_C}{P|_C}} & \leq \frac{8\gamma \log(B)}{R(C)}.
\end{align}
\end{theorem}
\begin{proof}
Observe that 
\label{eq:part1}
\begin{align*}
    \KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} &= \E_{\x \sim R|_C} \left[ \logf{R|_C(x)}{P|_C(x)} \right] - \E_{\x \sim R|_C} \left[ \logf{R|_C(x)}{Q|_C(x)} \right] = \E_{\x \sim R|_C} \left[\logf{Q_C(x)}{P_C(x)}\right],\\
    \KL{Q|_C}{P|_C} &= \E_{\x \sim  Q|_C}\left[\logf{Q|_C(x)}{P|_C(x)}\right].
\end{align*}
Letting 
\[ f(x) = \logf{Q|_C(x)}{P|_C(x)}\]
and subtracting, we  have
\begin{align}
    \label{eq:abs-exp}
    \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \KL{Q|_C}{P|_C}} = \abs{\E_{\x \sim  R|_C}[f(x)] - \E_{\x \sim  Q|_C}[f(x)]}.
\end{align}
Since $Q(x)/P(x)$ = $R(S)/P(S)$ for $S \ni x$,  
\[  f(x) := \logf{Q(x)P(C)}{Q(C)P(x)} = \logf{R(S)P(C)}{P(S)Q(C)} \]
hence $f \in \mFS$ since it is constant for each $S \in \mS$. We can bound $\infnorm{f}$ using Equation \eqref{eq:cons-3} as
\begin{align*} 
\|f|_\infty &= \max_{x \in \X} \abs{\logf{Q|_C(x)}{P|_C(x)}} \leq \max(\log(\infnorm{Q|_C/P|_C}), \log(\infnorm{P|_C/Q|_C})\\
& \leq \log(B^2) = 2\log(B). 
\end{align*}
We now apply Theorem \ref{thm:exp-bound} to the function $f$ to get
\begin{align}
    \abs{\E_{\x \sim  R|_C}[f(x)] - \E_{\x \sim  Q|_C}[f(x)]} \leq \frac{4\gamma}{R(C)} \infnorm{f} \leq \frac{8 \log(B)}{R(C)}.
\end{align}
Plugging this into Equation \eqref{eq:abs-exp} completes the proof.
\end{proof}





\subsection{Weakening the boundedness assumption}\label{sec:unbounded}

In this subsection, we show that the $B$-boundedness assumption is not needed for $\alpha$-multicalibration where $\beta = 0$. We show the following generalization of Theorem \ref{thm:pyth1}.





\begin{theorem}
\label{thm:pyth3}
Under Assumption \ref{asm:1} and the $B$-boundedness assumption, for any $C \in \mC$ we have
\begin{align}
    \label{eq:p-approx}
    \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \frac{Q(C)}{R(C)}\KL{Q|_C}{P|_C}} \leq      \hspace{4cm} \notag \\
\frac{1}{R(C)}\left(\alpha (\KL{R^\mS}{P^\mS} + 2)  + \beta\log(B) + \gamma \abs{\logf{P(C)}{Q(C)}}\right) .
\end{align}
\end{theorem}


The proof appears in Appendix \ref{app:weaken_bounded_proof}. A simple consequence of Theorem \ref{thm:pyth3} is that the $B$-boundedness assumption is not required under $\alpha$-multicalibration (i.e. $\beta =0$). 

\begin{corollary}
\label{thm:pyth2}
Under Assumption \ref{asm:1} with $\beta = 0$, for all $C \in \mC$ we have
\begin{align}
    \label{eq:p-simple1}
    \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \frac{Q(C)}{R(C)}\KL{Q|_C}{P|_C}}  \leq \frac{\alpha}{R(C)}\left(\KL{R^\mS}{P^\mS} + \abs{\logf{P(C)}{Q(C)}} + 2\right).
\end{align}
\end{corollary}




\eat{
If we had $Q(C) = R(C)$, then we could divide both sides by $R(C) = Q(C)$ to derive a bound on $\|E_{R|_C}[f] - \E_{Q|C}[f]$. While exact equality might not hold, we know $|R(C) - Q(C)|$ is small which lets us derive the following bound. 

\begin{lemma}
    Let $C \in \mC$, let $f \in \mFS$. Under Assumption \ref{asm:1}
    \begin{align}
    \label{eq:big-bound}
        \abs{\E_{\x \sim Q|_C}[f(x)]  - \E_{\x \sim R|_C}[f(x)]} \leq  
    \frac{1}{R(C)} \left(\alpha \E_{\x \sim R}[|f(\x)|] + (\alpha + \beta)\abs{\E_{\x \sim Q|_C}[f(\x)]} + \beta \|f\|_\infty\right)
    \end{align} 
\end{lemma}
\begin{proof}
    By the triangle inequality 
    \begin{align}
    \label{eq:triangle}
    R(C)\abs{\E_{\s \sim R|^\mS_C}[f(\s)] - \E_{\s \sim Q|^\mS_C}[f(\s)]} \leq
        \abs{R(C)\E_{\s \sim R|^\mS_C}[f(\s)] - Q(C)\E_{\s \sim Q|^\mS_C}[f(\s)]}
        + \abs{Q(C) - R(C)}\abs{\E_{\s \sim Q|^\mS_C}f(\s)}
    \end{align}
    We bound the first term using Lemma \ref{lem:omer}:
    \begin{align*}
        \abs{R(C)\E_{\s \sim R|^\mS_C}[f(\s)] - Q(C)\E_{\s \sim Q|^\mS_C}[f(\s)]} \leq  \alpha \E_{\x \sim R}[|f(\x)|] + \beta \|f\|_\infty.
    \end{align*}
    For the second term we use $|Q(C) - R(C)| \leq \alpha + \beta$ to get
    \begin{align*}
        \abs{Q(C) - R(C)}\abs{\E_{\s \sim Q|^\mS_C}[f(\s)]} \leq (\alpha + \beta)\abs{\E_{\s \sim Q|^\mS_C}[f(\s)]} = (\alpha + \beta)\abs{\E_{\x \sim Q|_C}[f(x)]}
    \end{align*}
    Substituting into Equation \eqref{eq:triangle} and dividing by $R(C)$, 
    \begin{align*} 
    \abs{\E_{\s \sim R|^\mS_C}[f(\s)] - \E_{\s \sim Q|^\mS_C}[f(\s)]} &\leq
\frac{1}{R(C)} \left(\alpha \E_{\x \sim R}[|f(\x)|] + (\alpha + \beta)\abs{\E_{\x \sim Q|_C}[f(x)]} + \beta \|f\|_\infty\right)\\
\end{align*}
\end{proof}



We now derive Theorem \ref{thm:pyth1} from Theorem \ref{thm:pyth3}. 
\begin{proof}[Proof of Theorem \ref{thm:pyth1}]
    We have
    \begin{align}
    \label{eq:big-bound}
        \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \KL{Q|_C}{P|_C}}  \leq &  
        \abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \frac{Q(C)}{R(C)}\KL{Q|_C}{P|_C}}\notag\\
        & + \abs{\frac{Q(C)}{R(C)} - 1}\KL{Q|_C}{P|_C}
    \end{align}
    We bound each term as a function of $\gamma$ and $\log(B)$. To bound the first  term, we apply Equation \eqref{eq:p-approx} from Theorem \ref{thm:pyth1} to get a bound of
    \begin{align}
    \label{eq:bound1}
        \frac{1}{R(C)}\left(\alpha (\KL{R^\mS}{P^\mS} + 2)  + \beta\log(B) + \gamma \abs{\logf{P(C)}{Q(C)}}\right) 
    \end{align}
    We use the boundedness assumption to bound the terms above in terms of $B$ as follows:
    \[ \frac{R^\mS(S)}{P^\mS(S)} = \frac{R(S)}{P(S)} \leq B.\]
    Hence $\KL{R^\mS}{P^\mS} \leq \log(B)$. Similarly
    \[ \frac{P(C)}{Q(C)} = \frac{\sum_{S \in \mS}P(S)P(C|S)}{\sum_{S \in \mS}R(S)P(C|S)}\]
    Since $P(S)/R(S) \in [1/B,B]$ it follows that $P(C)/Q(C)$ lies in the same range, hence
    \[ \abs{\logf{P(C)}{Q(C)}} \leq \log(B).\]
    Hence we can bound the first term in Equation \eqref{eq:big-bound} by 
    \begin{align}
    \label{eq:bound1.1}
        \frac{1}{R(C)}\left(\alpha (\KL{R^\mS}{P^\mS} + 2)  + \beta\log(B) + \gamma \abs{\logf{P(C)}{Q(C)}}\right) & \leq \frac{1}{R(C)}(\alpha(\log(B) + 2) + \beta\log(B) + \gamma \log(B) )\notag\\
        &\leq \frac{2\gamma (\log(B) + 2)}{R(C)}.
    \end{align}
    For the first term in Equation \eqref{eq:big-bound}, we have
    \[ \frac{Q|_C(x)}{P|_C(x)} = \frac{Q(x)P(C)}{P(x)Q(C)} \in(B^{-2}, B^2)\]
    hence $\KL{Q|_C}{P|_C} \leq 2\log(B)$. Since $|Q(C) - P(C)| \leq \gamma$,
    \[ \abs{Q(C) - R(C)}\KL{Q|_C}{P|_C} \leq 2\gamma \log(B).\]
    Plugging these in Equation \eqref{eq:bound1} gives 
    \[ 
    R(C)\abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \KL{Q|_C}{P|_C}} \leq 4 \gamma (\log(B) +1)
    \]
    Dividing by $R(C)$ gives the claimed bound. 
\end{proof}
 



}


==> results.tex <==
\section{Overview of Main Results}
\label{sec:results}

In this section we give a  technical overview of our results. Throughout we work under Assumption  \ref{asm:1}.

\iffalse
Let us recall the high level goals for computing the distribution $Q$. Firstly, $Q$ is a reweighing of $P$ such that the importance weights $w(x)$ could be estimated from samples of $R$ and $P$.  Secondly, we want $Q$ to serve as our model for $R$. The definitions of multiaccuracy and multicalibration formalize different ways in which $Q$ could be used in lieu of $R$. Roughly speaking, multiaccuracy means that every set $C \in \mC$ has similar measure under  $R$ and $Q$, while multicalibration states that $C$ could be partitioned according to $\mS$ and still $R$ and $Q$ assign similar measures to every partition of $C$ separately. It is natural to ask: what have we gained by having this additional guarantee, and how do we find a multi-calibrated partition? 
\fi
We start with the main technical tool we use.
For a partition $\mS$, let $\mFS$ denote the set of functions $f: \mS \rgta \R$. We can view these as functions $f: \X \rgta \R$ that are constant over sets $S \in \mS$. The most important example in this class is the weight function $w(x) = R(S)/P(S)$. Clearly, all functions of the form $f(x) = g(w(x))$ also belong to it.

\begin{theorem}\label{thm:main_informal}
	    Let $\mS$ be  partition of $\X$ and let $Q$ be a $(P, R, \mS)$-reweighted distribution over $\X$ that is $(\alpha,\beta)$-multicalibrated, then for every set $C \in \mC$ and $f \in \mFS$
		 \[ \abs{\E_{\x \sim Q|_C}[f(x)]  - \E_{\x \sim R|_C}[f(x)]} \leq  \frac{4\gamma \infnorm{f}}{R(C)}.\]
\end{theorem}

As an example, the case $f(x) = w(x)$ gives us Equation \eqref{eq:simple1} saying that the average anomaly scores under $R|_C$ are high, provided that $R(C)$ is sufficiently high. It is instructive to compare with Lemma~\ref{lem:exp-equal} that shows that for every partition, even not calibrated, it holds that 
$ \E_{\x \sim R}[f(\x)] = \E_{\x \sim Q}[f(\x)]$. The power of Theorem~\ref{thm:main_informal} lies in allowing conditioning on any $C \in \mC$.

\eat{
\paragraph{Anomaly Detection:} Here the importance weights are interpreted as anomaly scores. Recall that a high importance weight indicates that an item is more frequent in $R$ than in the prior $P$ and therefore is an anomaly. As we have argued, one cannot hope to identify anomalous points individually, but rather identify anomalous sets. Here $\mC$ denotes all sets of interest. Our goal therefore is that if a set $C$ is anomalous, i.e. $R(C)/P(C)$ is large, then the average anomaly score of points in $C$ would be large as well. First, some version of this is implied by multi-accuracy. Equation~\eqref{eq:ae} shows that
\[
\E_{x \sim P|_{C}}[w(x)] \in \E_{x \sim P|_{C}}[w(x^*)] \pm \frac{\alpha}{P(C)}.
\]
In other words, $\alpha$-multiAE guarantees that on expectation $w(x)$ is high where the expectation is taken over $P$. Our goal however is to bound the expectation under the real-world distribution $R$, since the objective is to find anomalies in $R$.
}
We can also derive a lower bound for the case when $\log(w(x))$ is used as the anomaly scores, which is the standard practice in anomaly detection algorithms. 

\begin{theorem}\label{thm:informal_anomaly}
	Under Assumptions \ref{asm:1} and \ref{asm:2}, for all $C \in \mC$ 
	such that $R(C) \geq 2\gamma$ we have
	\begin{equation} \nonumber
	\E_{\x \sim R|_C} [\log(w(x))] \geq  \logf{R(C)}{P(C)} - \gamma \frac{8\log(B) + 2}{R(C)}.
	\end{equation}
\end{theorem}
In addition, we prove similar bounds for other functions of the importance weights in Section~\ref{sec:anomaly}.

\eat{
Under mild assumptions multicalibration also implies a bound on the probability of a false positive, which is important because in practice a high false positive rate is the main drawback of many anomaly detection algorithms. Let $\tau$ be a threshold above which we consider a point to be an anomaly and let $S$ be the state marked as anomalous, therefore ${R(S)}/{P(S)} \geq \tau$. Let  $\delta > 0$ and $ C = \{ x: w^*(x) \leq \tau - \delta\}$ be the set of clearly normal points. With this setting we have the following bound:
\begin{theorem}
Assume $C\in \mC$, and $R(C)\ge 1/2$. Then under Assumption \ref{asm:1} with $R(S)\ge \beta$, the false positive rate $R(C|_S)$ is bounded as,
\[
R(C|_S) \leq \frac{2\tau\gamma}{\delta} + \frac{4\gamma}{R(S)}.
\]
\end{theorem}
}

\paragraph{Estimating the KL divergence:}
One of the main applications of importance weight estimation is to estimate the KL divergence between two distributions. The chain rule for KL divergence implies the following {\em Pythagorean theorem}.
\begin{lemma}
\label{lem:pyth-intro}
    Let $\mS$ be  partition of $\X$ and let $Q$ be the $(P, R, \mS)$-reweighted distribution over $\X$. Then
    \begin{equation}
        \label{eq:chain-r}
        \KL{R}{P} - \KL{R}{Q} = \KL{Q}{P}.
    \end{equation}
\end{lemma}
The lemma implies $\KL{Q}{P}$ is a lower bound for $\KL{R}{P}$, and further, since KL divergence is non-negative, the lower bound improves with the quality of the model. Note that the lemma does not require the partition to be multicalibrated.
With multicalibration, one can prove an approximate Pythagorean theorem for all conditonal distributions. 
 
\begin{theorem}
	Under Assumptions~\ref{asm:1}~and~\ref{asm:2}, for any $C \in \mC$ we have
	\begin{align}
	\label{eq:p-simple}
	\abs{\KL{R|_C}{P|_C} - \KL{R|_C}{Q|_C} - \KL{Q|_C}{P|_C}} & \leq \frac{8\gamma \log(B)}{R(C)}.
	\end{align}
\end{theorem}
An consequence that we discussed in the introduction is that the condition $\KL{Q|_C}{P|_C} \leq \KL{R|_C}{P|_C}$ holds approximately, so we do not overestimate the conditional divergence for any $C \in \mC$. 


\eat{
As we have seen, it might be the case that $Q$ and $R$ are very different distributions, and thus $\KL{R|_C}{P|_C}$ might be large, however, in our computational model we cannot distinguish between $Q$ and $R$ and so this divergence remains hidden. The theorem states that up to this hidden divergence and small error terms,  $\KL{Q|_C}{P|_C}$ approximates $\KL{R|_C}{P|_C}$. We stress again that this approximation holds for all subpopulations simultaneously. One does not need to sacrifice the accuracy of a subpopulation to get a good approximation overall. }

\paragraph{Algorithm for multicalibration}
Our main algorithmic contribution is an algorithm that computes a multicalibrated partition. The algorithm has access to $P$ and $R$ via samples and uses a weak agnostic learner for the concept class $\mC$ as a subroutine. 

The main idea of the algorithm is to iteratively modify a partition of the space, starting with the trivial partition of a single set which contains $\X$, until it arrives at a multicalibrated partition. Each iteration the algorithm applies one of two operations to the partition. The first operation uses the agnostic learner to check if it is beneficial to \emph{split} a set $S \subseteq \X$. We split the set if the learner finds $C \in \mC$ such that $\|P|_S(C) - R|_S(C)|$ is large. In this case the set is split to $S\cap C$ and $S \cap \bar C$. In the merge operation the algorithm  \emph{merges} sets of similar importance weight $R(S)/P(S)$, thus keeping the total size of the partition small. The algorithm terminates when the agnostic learner fails to split the partition further. The analysis is by showing that the KL divergence to $R$ goes on decreasing. The algorithm is reminiscent of boosting using branching programs \cite{mansour2002boosting,kalai2005boosting} in the supervised setting.



\eat{
To describe our guarantees for the algorithm, let $L$ be the number of samples required by the weak agnostic learner. We assume the $B$-boundedness condition (Assumption~\ref{asm:2}), and use $\tilde O(\cdot)$ to hide polynomial factors in $1/(\alpha \beta)$.
%We set $\alpha, \beta$ as targets for the multi-calibration, and use the $B$-boundedness assumption we use Assumption~\ref{asm:2}, and assume the agnostic learner needs $L$ samples. We use $\tilde O(\cdot)$ to hide polynomial factors in $1/(\alpha \beta)$.
	\begin{theorem}[informal]
     There is an algorithm that returns a partition $\mS$ that is $(\alpha, \beta)$-multicalibrated for $\mC$ under $P, R$. It runs for $T$ iterations where $T = \tilde O(\log(B)\KL{R}{P})$. It makes $O(T)$ calls to the weak agnostic learner, where each call requires $\tilde O(L\log B)$ samples from $R$ and $\tilde O(LB\log B)$ samples from $P$.
\end{theorem}
\iffalse
We show a second algorithm that only achieves multiaccuracy, but has lower complexity. It finds a multiaccurate distribution that is also a Gibbs distribution. Let $c$ be the indicator function of set $C$. The Gibbs distributions over $P$ are all distributions of the form 
\[ G(x) = P(x)\exp\left(\sum_{t=1}^T \lambda_t c_t(x) - \lambda_0\right) \]
where $c_t \in \mC$.  
Our algorithm learns an {\em unweighted} Gibbs distribution $Q$ where $\lambda_t =\eta$ for all $t$, hence the importance weights are of the form $w(x) = \exp(\eta\sum_{t=1}^T c_t(x))$. The algorithm is related to the well-known MaxEnt algorithm of \cite{dudik2007maximum}, and it can be viewed as solving a certain convex optimization problem using exponential updates/gradient descent. 

\begin{theorem}
    There is an algorithm that calls the agnostic learner $T \leq O(\KL{R}{P}/\alpha'^2)$ times and returns a Gibbs distribution $Q_T$ that is $\alpha$-multiaccurate.
\end{theorem}
\definecolor{}{}{}
}
